Accelerating Natural Gradient with Higher-Order Invariance

An appealing property of the natural gradient is that it is invariant to arbitrary differentiable reparameterizations of the model. However, this invariance property requires infinitesimal steps and is lost in practical implementations with small but finite step sizes. In this paper, we study invariance properties from a combined perspective of Riemannian geometry and numerical differential equation solving. We define the order of invariance of a numerical method to be its convergence order to an invariant solution. We propose to use higher-order integrators and geodesic corrections to obtain more invariant optimization trajectories. We prove the numerical convergence properties of geodesic corrected updates and show that they can be as computationally efficient as plain natural gradient. Experimentally, we demonstrate that invariance leads to faster optimization and our techniques improve on traditional natural gradient in deep neural network training and natural policy gradient for reinforcement learning.

==> ICML 2018 arXiv/abstract.tex <==
\begin{abstract}
%The efficacy of natural gradient method in training deep neural networks benefits from its invariance property of the update direction. Invariance under differentiable transformations makes the performance of algorithm independent of design choices. However, the update rule of natural gradient in the parameter space easily breaks invariance. In this paper, we examine the importance of invariance and propose to use higher-order integrators and geodesics on the model manifold to mitigate this problem. Experiments of training deep classifiers and autoencoders on several datasets show that respecting higher-order invariance gives favorable results. Our method can be directly used to accelerate natural gradient, and we believe it will provide valuable inspirations for other methods as well.

An appealing property of the natural gradient is that it is invariant to arbitrary differentiable reparameterizations of the model. However, this invariance property requires infinitesimal steps and is lost in practical implementations with small but finite step sizes. In this paper, we study invariance properties from a combined perspective of Riemannian geometry and numerical differential equation solving. We define the order of invariance of a numerical method to be its convergence order to an invariant solution. We propose to use higher-order integrators and geodesic corrections to obtain more invariant optimization trajectories. We prove the numerical convergence properties of geodesic corrected updates and show that they can be as computational efficient as plain natural gradient. Experimentally, we demonstrate that invariance leads to faster optimization and our techniques improve on traditional natural gradient in deep neural network training and natural policy gradient for reinforcement learning.
\end{abstract}

==> ICML 2018 arXiv/conclusion.tex <==
\section{Conclusion}
Our contributions in this paper can be summarized as:

\begin{itemize}[leftmargin=*]
	\item We propose to measure the invariance of numerical schemes by comparing their convergence to idealized invariant solutions.
	\item To the best of our knowledge, we are the first to use midpoint integrators for natural gradient optimization.
	\item Based on Riemannian Euler method, we introduce geodesic corrected updates. Moreover, the faster geodesic correction has comparable time complexity with vanilla natural gradient. Computationally, we also introduce new backpropagation type algorithms to compute connection-vector products. Theoretically, we provide convergence proofs for both types of geodesic corrected updates.
	\item Experiments confirm the benefits of invariance and demonstrate faster convergence and improved sample efficiency of our proposed algorithms in supervised learning and reinforcement learning applications.
\end{itemize}

For future research, it would be interesting to perform a thorough investigation over applications in reinforcement learning, and studying faster variants and more efficient implementations of the proposed acceleration algorithms.

\subsection*{Acknowledgements}
The authors would like to thank Jonathan McKinney for helpful discussions. This work was supported by NSF grants \#1651565, \#1522054, \#1733686, Toyota Research Institute, Future of Life Institute, and Intel.

%\section{Conclusion}

%Our goal is to accelerate natural gradient descent by preserving invariance. To this end, we propose two kinds of methods. The first one is based on a higher-order Runge-Kutta integrator, such as the midpoint method, to replace the natural gradient update. The second one is to use geodesics on the model manifold as a higher-order correction. The latter one has a faster variant, which can still lead to faster convergence than natural gradient when given the same time budget. 

%As for future directions, we plan to incorporate these acceleration methods into optimization algorithms derived from natural gradient, such as FANG~\cite{grosse2015scaling}, K-FAC~\cite{martens2015optimizing,grosse2016kronecker,badistributed} and unit-wise natural gradient~\cite{ollivier2013riemannian}. We are also actively seeking faster variants of midpoint integrator and more efficient ways of implementing acceleration algorithms.

==> ICML 2018 arXiv/experiments.tex <==
\section{Experimental Evaluations}
In this section, we demonstrate the benefit of respecting higher-order invariance through experiments on synthetic optimization problems, deep neural net optimization tasks and policy optimization in deep reinforcement learning.

Algorithms have abbreviated names in figures. We use ``\textbf{ng}'' to denote the basic natural gradient, ``\textbf{geo}'' to denote the one with geodesic correction, ``\textbf{geo\textsubscript{f}}'' to denote the faster geodesic correction, and ``\textbf{mid}'' to abbreviate natural gradient update using midpoint integrator. 


\subsection{Invariance}
In this experiment, we investigate the effect of invariance under different parameterizations of the same objective. We test different algorithms on fitting a univariate Gamma distribution via Maximum Log-Likelihood. The problem is simple---we can calculate the Fisher information metric and corresponding Levi-Civita connection accurately. Moreover, we can use ODE-solving software to numerically integrate the continuous natural gradient equation and calculate the exponential map used in Riemannian Euler method.

The pdf of Gamma distribution is 
\begin{equation*}
	p(x \mid \alpha, \beta) = \Gamma(x; \alpha, \beta) \triangleq \frac{\beta^\alpha}{\Gamma(\alpha)} x^{\alpha - 1} e^{-\beta x},
\end{equation*}
where $\alpha$, $\beta$ are shape and rate parameters. Aside from the original parameterization, we test three others: 1) $\alpha = \alpha', \beta = 1/\beta'$; 2) $\alpha = \alpha', \beta = (\beta')^3$ and 3) $\alpha = (\alpha')^2, \beta = (\beta')^2$, where $\alpha'$, $\beta'$ are new parameters. We generate 10000 synthetic data points from $\Gamma(X; 20, 20)$. During training, $\alpha$ and $\beta$ are initialized to 1 and the learning rate is fixed to 0.5. 

We summarize the results in \figref{fig:invariance}. Here ``\textbf{ng(exact)}'' is obtained by numerically integrating \eqref{eqn:ng}, and ``\textbf{geo(exact)}'' is obtained using Riemannian Euler method with a numerically calculated exponential map function. As predicted by the theory, both methods are exactly invariant under all parameterizations. From \figref{fig:invariance} we observe that the vanilla natural gradient update is not invariant under re-parameterizations, due to its finite step size. We observe that our midpoint natural gradient method and geodesic corrected algorithms are more resilient to re-parameterizations, and all lead to accelerated convergence of natural gradient.
% \begin{figure*}
% 	\centering
% 	\subfigure[]{
% 		\label{fig:midvsng}\includegraphics[width=0.3\textwidth]{ng-midpoint-thresh.png}
% 	}%
% 	\subfigure[]{
% 		\label{fig:geovsng}\includegraphics[width=0.3\textwidth]{ng-geo-thresh.png}
% 	}%
% 	\subfigure[]{
% 		\label{fig:geofvsng}\includegraphics[width=0.3\textwidth]{ng-fastgeo-thresh.png}
% 	}
	
% 	\caption{Robustness to hyper-parameters. Each cell corresponds to a hyper-parameter choice, and the color represents how much faster our method is compared to natural gradient in achieving $\alpha$ (white color means neither method succeeded in 1000 iterations).} 
% 	\label{fig:heatmap}
% \end{figure*}

\iffalse
\begin{figure*}
	\centering
	\vspace{-1.6eM}
% 	\subfigure[]{
% 		\label{fig:curves}
        \includegraphics[width=0.38\textwidth]{curves_all2.jpg}
% 	}%
% 	\subfigure[]{
% 		\label{fig:faces}
        \includegraphics[width=0.38\textwidth]{faces_all2.jpg}
% 	}%
	\vspace{-2eM}
% 	\subfigure[]{
% 		\label{fig:mnist}
        \includegraphics[width=0.38\textwidth]{mnist_all2.jpg}
% 	}%
% 	\subfigure[]{
% 		\label{fig:mnist_class}
        \includegraphics[width=0.38\textwidth]{mnist_class_all2.jpg}
% 	}%
	\vspace{-1eM}
	\caption{Training deep auto-encoders and classifiers with different acceleration algorithms. Solid lines show performance against number of iterations (bottom axis) while dashed lines depict performance against running time (top axis).} 
	\label{fig:deepencoder}	\label{fig:time}
\end{figure*}
\fi
\begin{figure*}
	\centering
	\includegraphics[width=0.8\textwidth]{fig.jpg}
	\caption{Training deep auto-encoders and classifiers with different acceleration algorithms. Solid lines show performance against number of iterations (bottom axes) while dashed lines depict performance against running time (top axes).} 	\label{fig:deepencoder}	\label{fig:time}
\end{figure*}

% \begin{figure*}
% 	\centering
% 	\vspace{-1.6eM}
%     \begin{subfigure}[t]{0.4\textwidth}
%     	\includegraphics[width=\textwidth]{curves_all2.jpg}
%         \label{fig:curves}
%     \end{subfigure}
% 	~
%     \begin{subfigure}[t]{0.4\textwidth}
%     	\includegraphics[width=\textwidth]{faces_all2.jpg}
%         \label{fig:faces}
%     \end{subfigure}
%     ~
%     \begin{subfigure}{0.4\textwidth}
%     	\includegraphics[width=\textwidth]{mnist_all2.jpg}
%         \label{fig:mnist}
%     \end{subfigure}
%    	~
%     \begin{subfigure}{0.4\textwidth}
%     	\includegraphics[width=\textwidth]{mnist_class_all2.jpg}
%         \label{fig:mnist_class}
%     \end{subfigure}
% 	\vspace{-1eM}
% 	\caption{Training deep auto-encoders and classifiers with different acceleration algorithms. Solid lines show performance against number of iterations (bottom axis) while dashed lines depict performance against running time (top axis).} 
% 	\label{fig:deepencoder}	\label{fig:time}
% \end{figure*}


\begin{figure*}
\centering
\includegraphics[width=0.9\textwidth]{acktr}
\caption{Sample efficiency of model-free reinforcement learning on continuous control tasks~\citep{todorov2012mujoco}. Titles indicate the environment used in OpenAI Gym~\citep{brockman2016openai}.}
\label{fig:acktr}
\end{figure*}

% \subsection{Synthetic Experiment: Robustness}
% For this experiment, we use the classical Rosenbrock function~\citep{rosenbrock1960automatic} to test the performance of the proposed algorithms. In order to add more complexity, we use a sum of 10 uncoupled 2D Rosenbrock functions. The optimization objective is defined as
% \begin{align*}
% f(\mbf{x}) \triangleq \sum_{i=1}^{10} [100 (x_{2i-1}^2 - x_{2i})^2 + (x_{2i -1} - 1)^2].
% \end{align*}

% We choose a relatively small-scale problem so that we can invert all metrics accurately. We also adopt a Levenberg-Marquardt style heuristic for adaptively choosing the damping coefficient when inverting matrices (see Appendix~\ref{app:settings}). In order to minimize the effect of confounding factors, we fix the initial parameters and learning rates for all algorithms. The only hyper-parameters we are considering are the two in the Marquardt heuristic for tuning the damping coefficient $\epsilon$: the $\epsilon$ increase factor when optimization gets stuck, and the $\epsilon$ decrease factor when optimization goes well~\citep{marquardt1963algorithm}. 

% %To use our framework, we convert $f(\mbf{x})$ to a probabilistic model $p_{\mbf{x}}(y) \sim \mcal{N}(\sqrt{f(\mbf{x})}; 1)$. Optimizing $f(\mbf{x})$ is then reduced to fitting $p_\mbf{x}(y)$ to a single sample $y = 0$. It is hard to measure the performance of each algorithm accurately. In this experiment, we approximately evaluate that by comparing the number of iterations needed to get $f(\mbf{x}) < \alpha$, where $\alpha$ is a predefined threshold.

% To study robustness to hyper-parameter settings, we provide heat maps in \figref{fig:heatmap} showing which method converges faster for various hyper-paramter choices. In this experiment, we approximately measure the convergence of algorithms by comparing the number of iterations needed to get $f(\mbf{x}) < \alpha$, where $\alpha$ is a predefined threshold. The color-coded value indicates how  much faster (number of iterations) our method achieves $\alpha=1$ compared to natural gradient (large is good). 
% %Here we choose $\alpha = 1$ as there are too few configurations that can achieve lower. 
% When neither method can achieve $\alpha$, the value is defined to be 0 (white). As the figures indicate, our acceleration methods can usually decrease faster than natural gradient under a larger fraction of hyper-parameter settings (but not always, as indicated by the blue squares).

% We first compare different algorithms under their individual best hyper-parameters. We did hyper-parameter tuning by enumerating a coarse grid of 100 values (more details in Appendix~\ref{app:exp}) and selecting configurations that achieve $\alpha = 0.1$ within the smallest number of iterations. The results are given in \figref{fig:best}, where we see that all our proposed acceleration methods can decrease much faster than natural gradient in the earlier stage of training. Comparatively, the difference in the later stage is not very significant since the values are already very small.

%\begin{figure}
%	\centering
%	\includegraphics[width=0.9\columnwidth]{best.png}\label{fig:best}
%	\caption{Comparing the speed of convergence of different algorithms on Rosenbrock function.}
%\end{figure}

\subsection{Training Deep Neural Nets}
We test our algorithms on deep autoencoding and classification problems. The datasets are CURVES, MNIST and FACES, all of which contain small gray-scale images of various objects, \ie, synthetic curves, hand-written digits and human faces. Since all deep networks use fully-connected layers and sigmoid activation functions, the tasks are non-trivial to solve even for modern deep learning optimizers, such as Adam~\cite{kingma2014adam}. Due to the high difficulty of this task, it has become a standard benchmark for neural network optimization algorithms~\citep{hinton2006reducing,martens2010deep,vinyals2012krylov,sutskever2013importance,martens2015optimizing}. Since these tasks only involve squared loss and binary cross-entropy, we additionally test multi-class cross-entropy on a MNIST classification task. Additional details can be found in Appendix~\ref{app:exp1}.

\figref{fig:deepencoder} summarizes our results on all three datasets. Here ``\textbf{ng}'' is the natural gradient method (Hessian-Free) as implemented in~\citet{martens2010deep}. For completeness, we also add Adam~\citep{kingma2014adam} into comparison and denote it as ``\textbf{adam}''. The training error reported for all datasets is the squared reconstruction error. Since the test error traces the training error very well, we only report the result of training error due to space limitation. It is clear that all acceleration methods lead to per iteration improvements compared to na\"{i}ve natural gradient. 
It is also remarkable that the performance of ``\textbf{geo\textsubscript{f}}'', while being roughly half as expensive as ``\textbf{geo}'' per iteration, does not degrade too much compared to ``\textbf{geo}''. For performance comparisons with respect to time, ``\textbf{geo\textsubscript{f}}'' is usually the best (or comparable to the best). ``\textbf{mid}'' and ``\textbf{geo}'' are relatively slower, since they need roughly twice as much computation per iteration as ``\textbf{ng}''. Nonetheless, ``\textbf{mid}'' still has the best time performance for MNIST classification task. 

We hereby emphasize again that geodesic correction methods are not aimed for providing more accurate solutions of the natural gradient ODE. Instead, they are higher-order approximations of an invariant solution (obtained by Riemannian Euler method), which itself is a first-order approximation to the exact solution. The improvements of both geodesic correction and midpoint integrator in \figref{fig:invariance} and \figref{fig:deepencoder} confirm our intuition that preserving higher-order invariance can accelerate natural gradient optimization.

%Algorithms turn out to perform similarly on the FACES dataset. This is probably because natural gradient keeps the invariance well and no much room can be explored by our acceleration methods. Also, the curves of FACES have a smooth trend of decreasing without any sign of getting trapped in saddle points~\cite{dauphin2014identifying}. This indicates that our acceleration methods might best suit problems with complicated loss landscapes. 

%It is also remarkable that the performance of ``\textbf{geo\textsubscript{f}}'', while being roughly half as expensive as ``\textbf{geo}'' per iteration, does not significantly degrade compared to ``\textbf{geo}''. This is natural since both of them correct the natural gradient update to the same order of error. 
%It will be even more evident when we show results for multi-class classification in the next section.

%\subsection{Deep classifier}
%\textbf{Deep classifier:} 
%The deep auto-encoder tasks only involve squared loss and binary cross-entropy loss. 
%In order to examine the performance of our algorithms for multi-class cross-entropy, we test them on a MNIST classification task. The network structure is 784-1000-500-250-30-10, all with fully connected layers. 
%The other hyper-parameters, such as maximum number of iterations of CG, maximum number of epochs, and damping threshold are all the same as those in the last section. 
%As preprocessing, we center and normalize all training and test data.
%The results are summarized in \figref{fig:mnist_class}. As expected, all acceleration methods improve the per iteration performance. The faster geodesic correction \textbf{geo\textsubscript{f}} works even better than \textbf{geo}. This problem seems to be especially suitable for midpoint integrator and \textbf{mid} is the only method that achieves 0 training error within 70 iterations.

%To demonstrate the time effectiveness of faster geodesic correction, we compare the per time performance of geo\textsubscript{f} with na\"{i}ve natural gradient on all tasks discussed so far. The results are shown in~\figref{fig:time}, where the unit of x-axis is second and ``MNIST class'' denotes the classification task on MNIST. The only dataset that \textbf{geo\textsubscript{f}} performs worse is FACES. This is already anticipated from~\figref{fig:deepencoder}, since no acceleration method leads to a significant improvement and the overhead of estimating connection renders \textbf{geo\textsubscript{f}} slow. For MNIST classification, the midpoint method \textbf{mid} performs so well that although it is several times more expensive to compute than natural gradient, it still gets the best result given limited time.

\subsection{Model-free Reinforcement Learning for Continuous Control}
Finally, we evaluate our methods in reinforcement learning over six continuous control tasks~\citep{todorov2012mujoco}. Specifically, we consider improving the algorithm of ACKTR~\citep{wu2017scalable}, an efficient variant of natural policy gradient~\citep{kakade2002natural} which uses Kronecker factors~\citep{martens2015optimizing} to approximately compute the inverse of Fisher information matrix. For these methods, we evaluate sample efficiency (expected rewards per episode reached within certain numbers of interactions); in robotics tasks the cost of simulation often dominates the cost of the reinforcement learning algorithm, so requiring less interactions to achieve certain performance has higher priority than lower optimization time per iteration. Therefore we only test midpoint integrator and geodesic correction method for improving ACKTR, and omit the faster geodesic correction because of its less accurate approximation.

Figure~\ref{fig:acktr} describes the results on the continuous control tasks, where we use ``\textbf{mid-}'' and ``\textbf{geo-}'' to denote our midpoint integrator and geodesic correction methods for ACKTR respectively. In each environment, we consider the same constant learning rate schedule for all three methods (detailed settings in Appendix~\ref{app:exp2}). While the Fisher information matrices are approximated via Kronecker factors, our midpoint integrator and geodesic correction methods are still able to outperform ACKTR in terms of sample efficiency in most of the environments. This suggests that preserving higher-order invariance could also benefit natural policy gradients in reinforcement learning, and our methods can be scaled to large problems via approximations of Fisher information matrices.

==> ICML 2018 arXiv/geocor.tex <==
\section{Geodesic Correction for Neural Networks}
Adding geodesic correction requires computing the Levi-Civita connection $\Gamma_{\mu\nu}^\alpha$ (see \eqref{eqn:connection}), which usually involves second-order derivatives. This is to the contrast of natural gradient, where the computation of Fisher information matrix only involves first-order derivatives of outputs. In this section, we address the computational issues of geodesic correction in optimizing deep neural networks.

%The invariance property of natural gradient is especially appealing to training deep neural networks. Traditional backpropagation is sensitive to factors like data representation, activation functions and scaling. It is generally recommended to normalize or even whiten input data. In addition, hyperbolic tangent functions are found to be better than logistic functions for centralizing network activities. \cite{lecun2012efficient} further proposes to use a specially scaled activation function $1.7159\tanh(2x/3)$ instead of $\tanh(x)$. All those tricky modifications correspond to potentially complex reparameterizations of the network. It would thus be interesting to have algorithms agnostic to arbitrary design choices.

In order to use natural gradient for neural network training, we first need to convert neural networks to probabilistic models. A feed-forward network can be treated as a conditional distribution $p_\theta(\mbf{t}\mid \mbf{x})$. For regression networks, $p_\theta(\mbf{t}\mid \mbf{x})$ is usually a family of multivariate Gaussians. For classification networks, $p_\theta(\mbf{t}\mid\mbf{x})$ usually becomes a family of categorical distributions. The joint probability density is $q(\mbf{x})p_\theta(\mbf{t}\mid\mbf{x})$, where $q(\mbf{x})$ is the data distribution and is usually approximated with the empirical distribution.

The first result in this section is the analytical formula of the Levi-Civita connection of neural networks.

\begin{proposition}
\label{analytic-levi}
	The Levi-Civita connection of a neural network model manifold is given by
	\begin{multline}
	\Gamma^\mu_{\alpha\beta} = g^{\mu\nu} \mbb{E}_{q(\mbf{x})} \mbb{E}_{p_\theta(\mbf{t}\mid\mbf{x})} \\\bigg\{ \partial_\nu \log p_\theta(\mbf{t}\mid\mbf{x})
	\bigg[ \partial_\alpha \partial_\beta \log p_\theta(\mbf{t}\mid\mbf{x}) +\\ \frac{1}{2}\partial_\alpha \log p_\theta(\mbf{t}\mid\mbf{x}) \partial_\beta \log p_\theta(\mbf{t}\mid\mbf{x})\bigg]\bigg\}
	\end{multline}
\end{proposition}
\begin{proof}
In Appendix~\ref{app:proofs}.
\end{proof}
%\begin{proof}
	%Let $r_\theta(\mbf{z})$ be the joint distribution defined by $q(\mbf{x})p_\theta(\mbf{t}\mid\mbf{x})$. The Fisher information metric is $g_{\mu\nu} = \mbb{E}_{\mbf{z}} [\partial_\mu \ln r_\theta(\mbf{z}) \partial_\nu \ln r_\theta(\mbf{z})]$. The partial derivative $\partial_\mu g_{\alpha\beta}$ can be computed via scoring function trick, \ie, $\partial_\mu g_{\alpha\beta} = \partial_\mu \mbb{E}_{\mbf{z}}[\partial_\alpha \ln r_\theta(\mbf{z})\partial_\beta \ln r_\theta(\mbf{z})] = \mbb{E}_\mbf{z}[\partial_\mu \ln r_\theta(\mbf{z}) \partial_\alpha \ln r_\theta(\mbf{z}) \partial_\beta \ln r_\theta(\mbf{z}) + \partial_\mu\partial_\alpha \ln r_\theta(\mbf{z}) \partial_\beta \ln r_\theta(\mbf{z})+\partial_\alpha \ln r_\theta(\mbf{z}) \partial_\mu \partial_\beta \ln r_\theta(\mbf{z})]$. All other partial derivatives can be obtained via symmetry.
	%
	%According to the definition, $\Gamma^\mu_{\alpha\beta} = \frac{1}{2} g^{\mu\nu} (\partial_\alpha g_{\nu\beta} + \partial_\beta g_{\nu\alpha} - \partial_\nu g_{\alpha\beta}) = g^{\mu\nu}\mbb{E}_{\mbf{z}}\big\{ \partial_\nu \ln r_\theta(\mbf{z}) \big[ \partial_\alpha\partial_\beta \ln r_\theta(\mbf{z}) + \frac{1}{2} \partial_\alpha \ln r_\theta(\mbf{z}) \partial_\beta \ln r_\theta(\mbf{z})\big]\big\}$. The proposition is proved after replacing $r_\theta(\mbf{z})$ with $q(\mbf{x})p_\theta(\mbf{t}\mid\mbf{x})$.
%\end{proof}

We denote the outputs of a neural network as $\mbf{y}(\mbf{x}, \theta) = (y_1,y_2,\cdots,y_o)$, which is an $o$-dimensional vector if there are $o$ output units. In this paper, we assume that $\mbf{y}(\mbf{x},\theta)$ are the values \emph{after} final layer activation (\eg, softmax). 
For typical loss functions, the expectation with respect to the corresponding distributions can be calculated analytically. Specifically, we instantiate the Levi-Civita connection for model distributions induced by three common losses and summarize them in the following proposition.

%\begin{proposition}\label{prop:l2}
	%For squared losses, the corresponding distribution is Gaussian, \ie, $p_\theta(\mbf{t}\mid\mbf{x}) = \prod_{i=1}^o \mcal{N}(t_i\mid y_i, \sigma^2)$. The Fisher information metric is  $g_{\mu\nu} = \frac{1}{\sigma^2} \sum_{i=1}^o \mbb{E}_{q(\mbf{x})}[\partial_\mu y_i \partial_\nu y_i]$ and the Levi-Civita connection has the form $\Gamma^\mu_{\alpha\beta} = \frac{1}{\sigma^2} \sum_{i=1}^o g^{\mu\nu} \mbb{E}_{q(\mbf{x})} [\partial_\nu y_i \partial_\alpha \partial_\beta y_i].$
%\end{proposition}
%\begin{proof}
	%In the appendix.
%\end{proof}
%\begin{proposition}\label{prop:logistic}
	%For binary cross-entropy losses, the corresponding distribution is Bernoulli distribution, \ie, $p_\theta(\mbf{t}\mid\mbf{x}) = \prod_{i=1}^o y_i^{t_i} (1 - y_i)^{1-t_i}$. The Fisher information metric is $g_{\mu\nu} = \sum_{i=1}^{o} \mbb{E}_{q(\mbf{x})} \bigg[ \frac{1}{y_i(1-y_i)}\partial_\mu y_i \partial_\nu y_i\bigg],$ and the Levi-Civita connection has the form $\Gamma^\mu_{\alpha\beta} = g^{\mu\nu} \sum_{i=1}^o \mbb{E}_{q(\mbf{x})}\bigg[ \frac{2y_i-1}{2y_i^2(1-y_i)^2} \partial_\nu y_i \partial_\alpha y_i \partial_\beta y_i + \frac{1}{y_i(1-y_i)}\partial_\nu y_i\partial_\alpha\partial_\beta y_i \bigg].$
%\end{proposition}
%\begin{proof}
	%In the appendix.
%\end{proof}
%\begin{proposition}\label{prop:softmax}
	%For multi-class cross-entropy losses, the corresponding distribution is categorical distribution, \ie, $p_\theta(\mbf{t}\mid\mbf{x}) = \prod_{i=1}^o y_i^{t_i}, \sum_{i=1}^o y_i = 1$. The Fisher information metric is $g_{\mu\nu} = \frac{1}{\sigma^2} \sum_{i=1}^o \mbb{E}_{q(\mbf{x})}\bigg[\frac{1}{y_i}\partial_\mu y_i \partial_\nu y_i\bigg]$ and the Levi-Civita connection has the form $\Gamma^\mu_{\alpha\beta} = g^{\mu\nu} \sum_{i=1}^o \mbb{E}_{q(\mbf{x})}\bigg[ \frac{1}{y_i} \partial_\nu y_i \partial_\alpha \partial_\beta y_i - \frac{1}{2y_i^2}\partial_\nu y_i \partial_\alpha y_i \partial_\beta y_i \bigg].$
%\end{proposition}
%\begin{proof}
	%In the appendix.
%\end{proof}


%\se{given that we have space, reformat the statement to be more readable}

\begin{proposition}\label{prop:l2}
%The Fisher information metrics and Levi-Civita connections can be computed as follows. 
For the squared loss, we have
\begin{align*}
p_\theta(\mbf{t}\mid\mbf{x}) &= \prod_{i=1}^o \mcal{N}(t_i \mid y_i, \sigma^2)\\
g_{\mu\nu} &= \frac{1}{\sigma^2} \sum_{i=1}^o \mbb{E}_{q(\mbf{x})}[\partial_\mu y_i \partial_\nu y_i]\\
\Gamma^\mu_{\alpha\beta} &= \frac{1}{\sigma^2} \sum_{i=1}^o g^{\mu\nu} \mbb{E}_{q(\mbf{x})} [\partial_\nu y_i \partial_\alpha \partial_\beta y_i]
\end{align*}
For the binary cross-entropy loss, we have 
\begin{align*}
p_\theta(\mbf{t}\mid \mbf{x}) &= \prod_{i=1}^o y_i^{t_i} (1-y_i)^{1-t_i}\\
g_{\mu\nu} &= \sum_{i=1}^{o} ~\mbb{E}_{q(\mbf{x})} \bigg[~\frac{1}{y_i(1-y_i)}\cdot\partial_\mu y_i \partial_\nu y_i~\bigg]\\
\Gamma^\mu_{\alpha\beta} &= g^{\mu\nu} \sum_{i=1}^o~ \mbb{E}_{q(\mbf{x})}\bigg[ ~\frac{2y_i-1}{2y_i^2(1-y_i)^2} \cdot \partial_\nu y_i \partial_\alpha y_i \partial_\beta y_i \\
&\qquad\qquad\qquad+ \frac{1}{y_i(1-y_i)}\cdot \partial_\nu y_i\partial_\alpha\partial_\beta y_i ~\bigg].
\end{align*}
In the case of multi-class cross-entropy loss, we have
\begin{align*}
p_\theta(\mbf{t}\mid\mbf{x}) &= \prod_{i=1}^o y_i^{t_i}\\
g_{\mu\nu} &= \frac{1}{\sigma^2} \sum_{i=1}^o~ \mbb{E}_{q(\mbf{x})}\bigg[\frac{1}{y_i}\cdot \partial_\mu y_i \partial_\nu y_i\bigg]\\
\Gamma^\mu_{\alpha\beta} &= g^{\mu\nu} \sum_{i=1}^o ~\mbb{E}_{q(\mbf{x})}\bigg[ \frac{1}{y_i} \cdot \partial_\nu y_i \partial_\alpha \partial_\beta y_i \\
&\qquad\qquad\qquad- \frac{1}{2y_i^2}\cdot \partial_\nu y_i \partial_\alpha y_i \partial_\beta y_i \bigg].
\end{align*}
\end{proposition}
\begin{proof}
	In Appendix~\ref{app:losses}.
\end{proof}
For geodesic correction, we only need to compute connection-vector products $\Gamma_{\alpha\beta}^\mu \dot{\gamma}^\alpha \dot{\gamma}^\beta$. This can be done with a similar idea to Hessian-vector products~\citep{pearlmutter1994fast}, for which we provide detailed derivations and pseudocodes in Appendix~\ref{app:computation}. It can also be easily handled with automatic differentiation frameworks. We discuss some practical considerations on how to apply them in real cases in Appendix~\ref{app:settings}.
\begin{figure*}
	\centering
	\includegraphics[width=0.95\textwidth]{gamma.png}
	\caption{The effect of re-parameterizations on algorithms fitting a univariate Gamma distribution. Titles indicate which parameterization was used.}\label{fig:invariance}
\end{figure*}
\section{Related Work}\label{sec:related}

The idea of using the geodesic equation to accelerate gradient descent on manifolds was first introduced in~\citet{transtrum2011geometry}. However, our geodesic correction has several important differences. Our framework is generally applicable to all probabilistic models. This is to be contrasted with ``geodesic acceleration'' in ~\citet{transtrum2011geometry} and \citet{transtrum2012geodesic}, which can only be applied to nonlinear least squares. Additionally, our geodesic correction is motivated from the perspective of preserving higher-order invariance, while in~\citet{transtrum2012geodesic} it is motivated as a higher-order correction to the Gaussian-Newton approximation of the Hessian under the so-called ``small-curvature assumption''. We discuss and evaluate empirically in Appendix~\ref{app:small} why the small-curvature approximation does not hold for training deep neural networks.

There has been a resurgence of interest in applying natural gradient to neural network training. \citet{martens2010deep}{ and \citet{martens2011learning} show that Hessian-Free optimization, which is equivalent to natural gradient method in important cases in practice~\citep{pascanu2013revisiting,martens2014new}, is able to obtain state-of-the-art results in optimizing deep autoencoders and RNNs. To scale up natural gradient, some approximations for inverting the Fisher information matrix have been recently proposed, such as Krylov subspace descent~\citep{vinyals2012krylov}, FANG~\citep{grosse2015scaling} and K-FAC~\citep{martens2015optimizing,grosse2016kronecker,badistributed}.

==> ICML 2018 arXiv/intro.tex <==
\section{Introduction}

Non-convex optimization is a key component of the success of deep learning. Current state-of-the-art training methods are usually variants of stochastic gradient descent (SGD), such as AdaGrad~\citep{duchi2011adaptive}, RMSProp~\citep{hintonlecture} and Adam~\citep{kingma2014adam}.
%These first-order optimizers can outperform plain SGD by exploiting diagonal approximations of the metric matrix. 
While generally effective, performance of those first-order optimizers is highly dependent on the curvature of the optimization objective. When the Hessian matrix of the objective at the optimum has a large condition number, the problem is said to have pathological curvature~\citep{martens2010deep,sutskever2013importance}, and first-order methods will have trouble in making progress. The curvature, however, depends on how the model is parameterized. There may be some equivalent way of parameterizing the same model which has better-behaved curvature and is thus easier to optimize with first-order methods. Model reparameterizations, such as good network architectures~\citep{simonyan2014very, he2016deep} and normalization techniques \citep{lecun2012efficient,ioffe2015batch,salimans2016weight} are often critical for the success of first-order methods.

The natural gradient~\citep{amari1998natural} method
%, although less widely adopted, 
takes a different perspective to the same problem. Rather than devising a different parameterization for first-order optimizers, it tries to make the optimizer itself invariant to reparameterizations by directly operating on the manifold of probabilistic models. %It relies only on intrinsic properties of this manifold, and is therefore invariant to model parameterizations, \eg, weight normalization and scalings in deep neural networks.
%
%There has been a resurgence of interest of applying natural gradient to neural network training. \cite{martens2010deep} show that Hessian-Free optimization, which is equivalent to natural gradient method in important cases in practice~\cite{pascanu2013revisiting,martens2014new} is able to obtain state-of-the-art results in optimizing deep autoencoders without pre-training. \cite{martens2011learning} further shows that the same Hessian-Free technique augmented with structural damping can train vanilla RNN efficiently, outperforming LSTMs~\cite{hochreiter1997long} in many difficult long-term dependency benchmarks. To scale up natural gradient, some approximations of inversing the Fisher information matrix have been recently proposed, such as Krylov subspace descent~\cite{vinyals2012krylov}, FANG~\cite{grosse2015scaling} and K-FAC~\cite{martens2015optimizing,grosse2016kronecker,badistributed}.
%
%Although there are many endeavors in adapting natural gradient method for deep learning and scaling up metric inverse calculations, little attention has been paid to the original update rule. The main selling point of natural gradient method, \emph{invariance} under differentiable transformations, actually only holds for continuous-time gradient trajectories~\cite{ollivier2013riemannian,ollivier2015riemannian}. In fact, the parameter update is only approximately invariant when the learning rate is very small. However, tiny learning rates hinter convergence. Inspired by Newton-Raphson method, the learning rate of natural gradient method is usually set to near 1 in real applications~\cite{martens2010deep,martens2014new}, which is far from being small. Such loss of invariance is a waste of the powerful differential geometric framework, and as demonstrated in the experiments, can often harm performance. 
This invariance, however, only holds in the idealized case of infinitesimal steps, \ie, for continuous-time natural gradient descent trajectories on the manifold~\citep{ollivier2013riemannian,ollivier2015riemannian}. Practical implementations with small but finite step size (learning rate) are only approximately invariant. 
%However, tiny learning rates hinder convergence. 
Inspired by Newton-Raphson method, the learning rate of natural gradient method is usually set to values near 1 in real applications~\citep{martens2010deep,martens2014new}, leading to potential loss of invariance. 
%Such loss of invariance is a waste of the powerful differential geometric framework, and as demonstrated in the experiments, can often harm performance. 

In this paper, we investigate invariance properties within the framework of Riemannian geometry and numerical differential equation solving. We observe that both the exact solution of the natural gradient dynamics and its approximation obtained with Riemannian Euler method~\citep{Bielecki2002-ix} are invariant. We propose to measure the invariance of a numerical scheme by \textit{studying its rate of convergence to those idealized truly invariant solutions}. It can be shown that the traditional natural gradient update (based on the forward Euler method) converges in first order. For improvement, we first propose to use a second-order Runge-Kutta integrator. Additionally, we introduce corrections based on the geodesic equation. We argue that the Runge-Kutta integrator converges to the exact solution in second order, and the method with geodesic corrections converges to the Riemannian Euler method in second order. Therefore, all the new methods have higher order of invariance, and experiments verify their faster convergence in deep neural network training and policy optimization for deep reinforcement learning. Moreover, the geodesic correction update has a faster variant which keeps the second-order invariance while being roughly as time efficient as the original natural gradient update. Our new methods can be used as drop-in replacements in any situation where natural gradient may be used.

%introduce two approaches to alleviate the loss of invariance and obtain a more accurate approximation of the truly invariant continuous-time gradient descent trajectory. Since the original update rule is equivalent to solving the natural gradient trajectory using first-order forward Euler method, we propose to improve it with a second-order Runge-Kutta integrator. In addition, inspired by the observation that geodesics are invariant to parameterization, we propose to use Riemannian Euler method~\cite{Bielecki2002-ix} instead of forward Euler update. From this point of view, the original update rule solves the geodesic equation to first order. Similar to~\cite{transtrum2011geometry}, we introduce a second-order correction derived from the geodesic equation. Experiments verify that this second-order term can boost convergence in a similar way to the second-order integrator. Furthermore, the second-order geodesic correction is more flexible and leads to an algorithm roughly as time efficient as the original natural gradient method.

==> ICML 2018 arXiv/invariance.tex <==
\input{midpoint}

\section{Riemannian Euler Method}
%Using higher-order integrators is not the only way for preserving higher-order invariance. As an example, 
For solving the natural gradient ODE (Eq.~\eqref{eqn:ng}), the Riemannian Euler method's update rule becomes%The solution obtained with this method is exactly invariant to reparameterizations. The update rule is given by
\begin{align}
	\theta_{k+1}^\mu = \operatorname{Exp}(\theta_{k}^\mu, -h\lambda g^{\mu\nu}\partial_\nu L(r_{\theta_k})), \label{eq:reuler}
\end{align}
where $\operatorname{Exp}:\{ (p,v)\mid p\in \mcal{M}, v\in \mcal{T}_p\mcal{M} \}\rightarrow \mcal{M}$ is the exponential map as defined in \secref{sec:pre}. The solution obtained by Riemannian Euler method is invariant to reparameterizations, because $\operatorname{Exp}$ is a function independent of parameterization and for each step, the two arguments of $\operatorname{Exp}$ are both invariant. 

%The first argument $\theta_k^\mu$ denotes current position on the manifold, and the second argument $-h\lambda g^{\mu\nu}\partial_\nu L$ is a vector in the current tangent space. $\operatorname{Exp}$ takes in those two arguments, follows a geodesic on the manifold, and gives the next position. Each step of update is thus invariant since geodesics are intrinsic to the manifold (as illustrated in \figref{fig:paths}), and the optimization procedure composed of those invariant segments is also invariant.

\subsection{Geodesic Correction}
%There is also an alternative way to explain the loss of invariance of the update $\theta_{t+1} \gets \theta_t - \eta g^{\mu\nu}\partial_\nu l$. The natural gradient direction $g^{\mu\nu}\partial_\nu l$ is invariant, and we assume it is a good direction to follow. However, moving along a straight line in the parameter space, which is what the old update rule does, will not yield a straight trajectory in the model space. Actually, the trajectory in the model space corresponding to a linear update in the parameter space will typically veer away from a straight line. This distortion from a straight line is both parameterization-dependent and unnatural for optimization.

For most models, it is not tractable to compute $\operatorname{Exp}$, since it requires solving the geodesic equation \eqref{eq:geo} exactly. Nonetheless, there are two numerical methods to approximate geodesics, with different levels of accuracy. 

According to \secref{sec:pre}, 
$\operatorname{Exp}(\theta_k^\mu, -h \lambda  g^{\mu\nu}\partial_\nu L(r_{\theta_k})) = \gamma^\mu_k(h)$, where $\gamma^\mu_k$ satisfies the geodesic equation \eqref{eq:geo} and
\begin{align*}
\gamma^\mu_k(0) &= \theta_k^\mu \\
\dot\gamma^\mu_k(0) &= - \lambda g^{\mu\nu} \partial_\nu L(r_{\theta_k}).
\end{align*}
The first method for approximately solving $\gamma^\mu_k(t)$ ignores the whole geodesic equation and only uses information of first derivatives, giving $$\gamma_k^\mu(h) \approx \theta_{k}^\mu + h \dot{\gamma}^\mu_k(0) = \theta_k^\mu - h \lambda g^{\mu\nu}\partial_\nu L,$$which corresponds to the na\"{i}ve natural gradient update rule. 

The more accurate method leverages information of second derivatives from the geodesic equation~\eqref{eq:geo}. The result is 
\begin{align*}
\gamma^\mu_k(h) &\approx \theta^\mu_k + h \dot{\gamma}_k^\mu(0) + \frac{1}{2}h^2 \ddot{\gamma}^\mu_k(0)\\
 &= \theta^\mu_k - h \lambda g^{\mu\nu}\partial_\nu L - \frac{1}{2}h^2 \Gamma^{\mu}_{\alpha\beta} \dot{\gamma}_k^\alpha(0) \dot{\gamma}_k^\beta(0).
\end{align*}
The additional second-order term given by the geodesic equation (\ref{eq:geo})  reduces the truncation error to third-order. This corresponds to our new natural gradient update rule with \emph{geodesic correction}, \ie, 
\begin{align}
\theta_{k+1}^\mu = \theta_{k}^\mu + h \dot{\gamma}^\mu_k(0) - \frac{1}{2}h^2 \Gamma^\mu_{\alpha\beta} \dot{\gamma}^\alpha_k(0) \dot{\gamma}^\beta_k(0),\label{main:geo:eq}
\end{align}
where $\dot{\gamma}^\mu_k(0) = -\lambda g^{\mu\nu}\partial_\nu L(r_{\theta_k})$. 

%The update rule $\theta_{t+1} \gets \theta_t - h\lambda g^{\mu\nu}\partial_\nu l$ corresponds to moving along a straight line in the parameter space $\Theta$. In general, this will \emph{not} yield a straight trajectory in the model space $\mcal{M}$, as illustrated in \figref{fig:paths}.
%Actually, the trajectory in the model space corresponding to a linear update in the parameter space will typically veer away from a straight line. This distortion is both parameterization-dependent and unnatural for optimization.

%\subsubsection{The main idea}

% To solve this problem, we propose to follow straight lines in the model space, which are geodesics. Specifically, at each step we calculate the natural gradient direction for the current parameters and then parallel transport the direction vector along itself for a finite step size.
% and repeat this procedure for the next time step. 
% By parallel transporting the gradient, the trajectory of parameters will trace a geodesic line in the model space, which can be computed from the geodesic equation~\eqref{eq:geo}. 
%The geodesic equation is a second-order initial value problem with $\theta^\mu(0) = \theta_t^\mu, \dot \theta^\mu(0) = -g^{\mu\nu}\partial_\nu l$ and our target is to solve $\ddot \theta^\mu + \Gamma^\mu_{\alpha\beta}\dot{\theta^\alpha}\dot{\theta^\beta} = 0$ for $\theta(\eta)$. 
%This is a second-order ODE $\ddot \theta^\mu + \Gamma^\mu_{\alpha\beta}\dot{\theta^\alpha}\dot{\theta^\beta} = 0$ with initial conditions $\theta^\mu(0) = \theta_t^\mu, \dot \theta^\mu(0) = -\lambda g^{\mu\nu}\partial_\nu l$. Our goal is to solve for $\theta(t)$. 

%When $h$ is small, there are two numerical solutions with different degrees of accuracy. 

%The first one ignores the whole geodesic equation and only uses the initial values, giving $\theta^\mu(h) = \theta^\mu(0) - h \lambda g^{\mu\nu}\partial_\nu l$. This corresponds to the na\"{i}ve update rule of natural gradient method and has an error up to second-order. The second one uses both the geodesic equation and initial values. The result is $\theta^\mu(h) = \theta^\mu(0) + h \dot{\theta}^\mu(0) + \frac{1}{2}h^2 \ddot{\theta}^\mu(0) = \theta^\mu(0) - h \lambda g^{\mu\nu}\partial_\nu l - \frac{1}{2}h^2 \Gamma^{\mu}_{\alpha\beta} \dot{\theta}^\alpha(0) \dot{\theta}^\beta(0)$. The additional second-order term from the geodesic equation reduces the numerical error to third-order. This corresponds to our new natural gradient update rule with \emph{geodesic correction}, \ie, 
%\begin{align}
%\label{main:geo:eq}
%\theta_{t+1}^\mu \gets \theta_{t}^\mu + h \dot{\theta}^\mu_t - \frac{1}{2}h^2 %\Gamma^\mu_{\alpha\beta} \dot{\theta}^\alpha_t \dot{\theta}^\beta_t,
%\end{align}
%where $\dot{\theta}^\mu_t = -\lambda g^{\mu\nu}_t\partial_\nu l$. 
%\se{eq is missing some $t$ subscripts}


\subsection{Faster Geodesic Correction}

To obtain the second order term in the geodesic corrected update, we first need to compute $\dot{\gamma}_k(0)$, which requires inverting the Fisher information matrix. Then we have to plug in $\dot{\gamma}_k(0)$ and compute $\Gamma^\mu_{\alpha\beta}\dot{\gamma}_k^\alpha(0) \dot{\gamma}_k^\beta(0)$, which involves inverting the same Fisher information matrix again (see \eqref{eqn:connection}). Matrix inversion (more precisely, solving the corresponding linear system) is expensive and it would be beneficial to combine the natural gradient and geodesic correction terms together and do only one inversion.

To this end, we propose to estimate $\dot\gamma_k(0)$ in $\Gamma_{\alpha\beta}^\mu \dot{\gamma}_k(0)^\alpha \dot{\gamma}_k(0)^\beta$ with $\dot\gamma_k(0) \approx (\theta_k - \theta_{k - 1})/h$. 
Using this approximation and substituting (\ref{eqn:connection}) into (\ref{main:geo:eq}) gives the following faster geodesic correction update rule:
\begin{align}
\delta\theta_{k}^\mu &= \lambda g^{\mu\nu}\cdot
\bigg[ -\partial_\nu L(r_{\theta_k}) - 
\\ &\frac{1}{4} h\lambda (\partial_\alpha g_{\nu\beta} + \partial_\beta g_{\nu\alpha} - \partial_\nu g_{\alpha\beta})\delta\theta_{k-1}^\alpha\delta\theta_{k-1}^\beta\bigg] \nonumber\\
\theta_{k+1}^\mu &= \theta_{k}^\mu +h\delta\theta_{k}^\mu,\label{main:fastergeo:eq}
\end{align}
which only involves one inversion of the Fisher information matrix. 

\subsection{Convergence Theorem}
We summarize the convergence properties of geodesic correction and its faster variant in the following general theorem.
\begin{theorem}[Informal]\label{thm:converge}
	Consider the initial value problem $\dot x = f(t, x(t)), x(0) = a, 0\leq t \leq T$. Let the interval $[0, T]$ be subdivided into $n$ equal parts by the grid points $0 = t_0 < t_1 < \cdots < t_n = T$, with the grid size $h = T / n$. Denote $x_k$ and $\hat{x}_k$ as the numerical solution given by geodesic correction and its faster version respectively.	Define the error $e_k$ at each grid point $x_k$ by $e_k = x_k' - x_k$, and $\hat{e}_k = x_k' - \hat{x}_k$, where $x_k'$ is the numerical solution given by Riemannian Euler method. Then it follows that
	\begin{equation*}
	\norm{e_k} \leq \mcal{O}(h^2)\quad \text{and} \quad	\norm{\hat{e}_k} \leq \mcal{O}(h^2),  h \rightarrow 0,  \forall k \in [n].
	\end{equation*}
	As a corollary, both Euler's update with geodesic correction and its faster variant converge to the solution of ODE in 1st order.
\end{theorem}
\begin{proof}
	Please refer to Appendix~\ref{app:proofs} for a rigorous statement and detailed proof.
\end{proof}

The statement of \thmref{thm:converge} is general enough to hold beyond the natural gradient ODE (Eq.~\eqref{eqn:ng}). It shows that both geodesic correction and its faster variant converge to the invariant Riemannian Euler method in 2nd order. In contrast, vanilla forward Euler method, as used in traditional natural gradient, is a first order approximation of Riemannian Euler method. In this sense, geodesic corrected updates preserve higher-order invariance.
%\input{midpoint}


==> ICML 2018 arXiv/midpoint.tex <==
\section{Higher-order Integrators}
%In this section, we discuss approaches to help alleviate the loss of invariance problem of natural gradient method. Specifically, we propose to use midpoint method, which is a second-order Runge-Kutta integrator, to solve the learning trajectory equation of natural gradient, \ie, $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$. We also exploited the invariance property of parallel transportation and suggest using geodesics to correct invariance loss of the na\"{i}ve update rule.

%\subsection{Midpoint integrator}

If we could integrate the learning trajectory equation $\dot \theta^\mu = - \lambda g^{\mu\nu}\partial_\nu L$ exactly, the optimization procedure would be invariant to reparameterizations. %.all differentiable parameterizations of the model. 
%This is especially appealing to training neural networks because of the superior representation power of neural models and its susceptibility to design choices. 
However, the na\"{i}ve linear update of natural gradient $\theta_{k+1}^\mu = \theta_k^\mu - h\lambda g^{\mu\nu}\partial_\nu L$ is only a forward Euler approximation, %As shown by blue arrows in \figref{fig:paths}, and linear updates in different parameter spaces can have parameterization-dependent deviations in the model manifold.
and can only converge to the invariant exact solution in first order.
Therefore, a natural improvement is to use higher-order integrators to obtain a more accurate approximation to the exact solution.
%trajectory with less error in order to capture higher-order invariance, and we propose to use midpoint integrator.

As mentioned before, the midpoint integrator has second-order convergence and should be generally more accurate. In our case, it becomes
%Adapted to the natural gradient context, the update rule now becomes 
\begin{align*}
\theta_{k+\frac{1}{2}}^\mu &= \theta_k^\mu
 - \frac{1}{2}h\lambda g^{\mu\nu}(\theta_k)\partial_\nu L(r_{\theta_k}),\\
\theta_{k+1}^\mu &= \theta_k^\mu - h\lambda g^{\mu\nu}(\theta_{k+\frac{1}{2}}) \partial_\nu L(r_{\theta_{k+\frac{1}{2}}}).
\end{align*}
%Here we let
%\begin{align*}
%g_{\mu\nu,t} &= \mbb{E}_{p_{\theta_t}(\mbf{z})}[\partial_\mu \ln p_{\theta_t}(\mbf{z})\partial_\nu \ln p_{\theta_t}(\mbf{z})]\\
%g_{\mu\nu,t+\frac{1}{2}} &= \mbb{E}_{p_{\theta_{t+\frac{1}{2}}}(\mbf{z})}[\partial_\mu \ln p_{\theta_{t+\frac{1}{2}}}(\mbf{z})\partial_\nu \ln p_{\theta_{t+\frac{1}{2}}}(\mbf{z})]\\
%\end{align*}
%and $g^{\mu\nu}_t, g^{\mu\nu}_{t+\frac{1}{2}}$ represent the inverses of $g_{\mu\nu,t}, g_{\mu\nu,t+\frac{1}{2}}$ respectively. 
where $g^{\mu\nu}(\theta_k), g^{\mu\nu}(\theta_{k+\frac{1}{2}})$ are the inverse metrics evaluated at $\theta_k$ and $\theta_{k+\frac{1}{2}}$ respectively. Since our midpoint integrator converges to the invariant natural gradient ODE solution in second order, it preserves higher-order invariance compared to the first-order Euler integrator used in vanilla natural gradient.

%The implementation of the midpoint integrator is straightforward. 
%Actually, only a small number of modifications is necessary for the original natural gradient update rule. 
%We calculate the natural gradient direction as usual, but use half of the regular step size $h/2$ to obtain an intermediate value $\theta_{k+\frac{1}{2}}$. Then we use the intermediate parameters to calculate a new natural gradient direction and use it to do an update with full step size $h$ to obtain $\theta_{k+1}$. Note that a midpoint integrator step is roughly twice as expensive as a traditional natural gradient method, but is more accurate. 

%One may propose to use linear multistep integrators such as Adams-Bashforth, since they are higher-order methods with a comparable computational cost to forward Euler, while Runge-Kutta methods are usually more expensive. We prefer Runge-Kutta methods over linear multistep counterparts because explicit multistep methods typically have very small regions of absolute stability~\cite{leveque2007finite}, which means in practice only very small step sizes can work.

%By using midpoint integrator, we expect the natural gradient update to have smaller error, thus being closer to the invariant solution of the ODE. We validate this empirically in later sections.

==> ICML 2018 arXiv/new_preliminaries.tex <==
\section{Preliminaries}
\subsection{Riemannian Geometry and Invariance}\label{sec:pre}

We use \emph{Einstein's summation convention} throughout this paper to simplify formulas. The convention states that when any index variable appears twice in a term, once as a superscript and once as a subscript, it indicates summation of the term over all possible values of the index variable. For example, $a^\mu b_\mu \triangleq \sum_{\mu=1}^n a^\mu b_\mu$ when index variable $\mu \in [n]$. 

Riemannian geometry is used to study intrinsic properties of differentiable manifolds equipped with metrics. The goal of this necessarily brief section is to introduce some key concepts related to the understanding of invariance. For more details, please refer to~\cite{petersen2006riemannian} and~\cite{amari1987differential}.

\begin{figure}
	\centering
		\includegraphics[width=0.95\columnwidth]{tangent_plane_plot.jpg}
	\caption{An illustration of Riemannian geometry concepts: tangent spaces, cotangent spaces, coordinate basis, dual coordinate basis, geodesics and the exponential map.}
	\label{fig:geometry}
\end{figure}

In this paper, we describe a family of probabilistic models as a manifold. Roughly speaking, a \emph{manifold} $\mcal{M}$ of dimension $n$ is a smooth space whose local regions resemble $\mbb{R}^n$~\citep{carroll2004spacetime}. Assume there exists a smooth mapping $\phi:\mcal{M}\rightarrow \mbb{R}^n$ in some neighborhood of $p$ and for any $p\in\mcal{M}$, $\phi(p)$ is the coordinate of $p$. As an example, if $p$ is a parameterized distribution, $\phi(p)$ will refer to its parameters. There is a linear space associated with each $p \in \mcal{M}$ called the \emph{tangent space} $\mcal{T}_p\cal{M}$. Each element $v \in \mcal{T}_p\cal{M}$ is called a \emph{vector}. For any tangent space $T_p \mcal{M}$, there exists a dual space $T_p^* \mcal{M}$ called the \emph{cotagent space}, which consists of all linear real-valued functions on the tangent space. Each element $v^*$ in the dual space $T_p^* \mcal{M}$ is called a \emph{covector}.  
Let $\phi(p) = (\theta^1,\theta^2,\cdots,\theta^n)$ be the coordinates of $p$, it can be shown that the set of operators $\{\frac{\partial}{\partial \theta^1},\cdots,\frac{\partial}{\partial \theta^n}\}$ forms a basis for $\mcal{T}_p\mcal{M}$ and is called the \emph{coordinate basis}. Similarly, the dual space admits the \emph{dual coordinate basis} $\{\ud\theta^1,\cdots,\ud\theta^n\}$. These two sets of bases satisfy $\ud\theta^\mu(\partial_\nu) = \delta^\mu_\nu$ where $\delta^{\mu}_\nu \triangleq \begin{cases}
1, \mu = \nu\\
0, \mu \neq \nu
\end{cases}$ is the Kronecker delta. Note that in this paper we abbreviate $\frac{\partial}{\partial \theta^\mu}$ to $\partial_\mu$ and often refer to an entity (\eg, vector, covector and point on the manifold) with its coordinates.

Vectors and covectors are geometric objects associated with a manifold, which exist independently of the coordinate system. However, we rely on their \textbf{representations} \wrt some coordinate system for quantitative studies. Given a coordinate system, a vector $\mbf{a}$ (covector $\mbf{a}^*$) can be represented by its coefficients \wrt the coordinate (dual coordinate) bases, which we denote as $a^\mu$ ($a_\mu$). Therefore, these coefficients depend on a specific coordinate system, and will change for different parameterizations. In order for those coefficients to represent coordinate-independent entities like vectors and covectors, their change should obey some appropriate transformation rules. Let the new coordinate system under a different parameterization be $\phi'(p) = (\xi^1,\cdots,\xi^n)$ and let the old one be $\phi(p) = (\theta^1,\cdots,\theta^n)$. It can be shown that the new coefficients of $\mbf{a} \in \mcal{T}_p\mcal{M}$ will be given by 
$
 a^{\mu'} = a^\mu \frac{\partial \xi^{\mu'}}{\partial \theta^\mu},
$
while the new coefficients of $\mbf{a}^* \in \mcal{T}_p^*\mcal{M}$ will be determined by 
$
a_{\mu'} = a_\mu \frac{\partial \theta^\mu}{\partial \xi^{\mu'}}.
$
Due to the difference of transformation rules, we say $a^\mu$ is \emph{contravariant} while $a_\mu$ is \emph{covariant}, as indicated by superscripts and subscripts respectively. In this paper, we only use Greek letters to denote contravariant / covariant components.

Riemannian manifolds are equipped with a positive definite metric tensor $g_p \in \mcal{T}_p^* \mcal{M} \otimes \mcal{T}_p^* \mcal{M}$, so that distances and angles can be characterized. The inner product of two vectors $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, $\mbf{b} = b^\nu \partial_\nu \in \mcal{T}_p\mcal{M}$ is defined as $\langle \mbf{a}, \mbf{b} \rangle \triangleq g_p(\mbf{a}, \mbf{b}) = g_{\mu\nu} \ud\theta^\mu \otimes \ud\theta^\nu (a^\mu \partial_\mu, b^\nu\partial_\nu) = g_{\mu\nu} a^\mu b^\nu$. For convenience, we denote the inverse of the metric tensor as $g^{\alpha\beta}$ using superscripts, \ie, $g^{\alpha\beta} g_{\beta\mu} = \delta^\alpha_\mu$. The introduction of inner product induces a natural map from a tangent space to its dual space. Let $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, its natural correspondence in $\mcal{T}_p^*\mcal{M}$ is the covector $\mbf{a}^* \triangleq \langle \mbf{a}, \cdot \rangle = a_\nu d\theta^\nu$. It can be shown that $a_\nu = a^\mu g_{\mu\nu}$ and $a^\mu = g^{\mu\nu}a_\nu$. We say the metric tensor relates the coefficients of a vector and its covector by lowering and raising indices, which effectively changes the transformation rule.

The metric structure makes it possible to define \emph{geodesics} on the manifold, which are constant speed curves $\gamma: \mbb{R} \rightarrow \mcal{M}$ that are locally distance minimizing. Since the distances on manifolds are independent of parameterization, geodesics are invariant objects. Using a specific coordinate system, $\gamma(t)$ can be determined by solving the \emph{geodesic equation}
\begin{align}
\ddot \gamma^\mu + \Gamma_{\alpha\beta}^\mu \dot\gamma^\alpha \dot \gamma^\beta = 0\label{eq:geo},
\end{align}
where $\Gamma_{\alpha\beta}^\mu$ is the \emph{Levi-Civita connection} defined by
\begin{align}
\Gamma_{\alpha\beta}^\mu \triangleq \frac{1}{2} g^{\mu\nu}(\partial_\alpha g_{\nu\beta} + \partial_\beta g_{\nu\alpha} - \partial_\nu g_{\alpha\beta}).\label{eqn:connection}
\end{align}
Note that we use $\dot{\gamma}$ to denote $\frac{\ud \gamma}{\ud t}$ and $\ddot{\gamma}$ for $\frac{\ud^2 \gamma}{\ud t^2}$.


Given $p\in\mcal{M}$ and $v \in \mcal{T}_p\mcal{M}$, there exists a unique geodesic satisfying $\gamma(0)=p, \dot{\gamma}(0) = v$. If we follow the curve $\gamma(t)$ from $p = \gamma(0)$ for a unit time $\Delta t = 1$, we can reach another point $p' = \gamma(1)$ on the manifold. In this way, traveling along geodesics defines a map from $\mcal{M} \times \mcal{T}\mcal{M}$ to $\mcal{M}$ called \emph{exponential map}
\begin{align}
\operatorname{Exp}(p,v) \triangleq \gamma(1),
\end{align}
where $\gamma(0) = p$ and $\dot{\gamma}(0) = v$. By simple re-scaling we also have $\operatorname{Exp}(p, h v) = \gamma(h)$.

As a summary, we provide a graphical illustration of relevant concepts in Riemannian geometry in~\figref{fig:geometry}. %From the above formulation, we observe that every concept and relation is defined via coordinates or coefficients. However, 
Here we emphasize again the important ontological difference between an object and its coordinate. The manifold itself, along with geodesics and vectors (covectors) in its tangent (cotangent) spaces is intrinsic and independent of coordinates. The coordinates need to be transformed correctly to describe the same objects and properties on the manifold under a different coordinate system. This is where invariance emerges.

\subsection{Numerical Differential Equation Solvers}
Let the ordinary differential equation (ODE) be
$\dot{x}(t) = f(t, x(t))$, where $x(0) = a$ and $t \in [0, T]$. Numerical integrators try to trace $x(t)$ with iterative local approximations $\{x_k \mid k\in\mbb{N}\}$.

We discuss several useful numerical methods in this paper. The forward Euler method updates its approximation by $x_{k+1} = x_k + h f(t_k, x_k)$ and $t_{k+1} = t_{k} + h$. It can be shown that as $h\rightarrow 0$, the error $\norm{x_k - x(t_k)}$ can be bounded by $\mcal{O}(h)$. The midpoint integrator is a Runge-Kutta method with $\mcal{O}(h^2)$ error. Its update formula is given by $x_{k+1} = x_k + h f\left( t_k + \frac{1}{2} h ,x_k + \frac{h}{2}f(t_k,x_k) \right)$, $t_{k+1} = t_{k} + h$. The Riemannian Euler method (see pp.3-6 in~\cite{Bielecki2002-ix}) is a less common variant of the Euler method, which uses the Exponential map for its updates as $x_{k+1} = \operatorname{Exp}(x_k,h f(t_k, x_k))$, $t_{k+1} = t_{k} + h$. While having the same asymptotic error $\mcal{O}(h)$ as forward Euler, it has more desirable invariance properties.


\subsection{Revisiting Natural Gradient Method}
Let $r_\theta(\mbf{x}, \mbf{t}) = p_\theta(\mbf{t}\mid\mbf{x})q(\mbf{x})$ denote a probabilistic model parameterized by $\theta \in \Theta$, where $\mbf{x},\mbf{t}$ are random variables, $q(\mbf{x})$ is the marginal distribution of $\mbf{x}$ and assumed to be fixed. Conventionally, $\mbf{x}$ is used to denote the input and $\mbf{t}$ represents its label. In a differential geometric framework, the set of all possible probabilistic models $r_\theta$ constitutes a manifold $\mcal{M}$, and the parameter vector $\theta$ provides a coordinate system. Furthermore, the infinitesimal distance of probabilistic models can be measured by the Fisher information metric $g_{\mu\nu} = \mbb{E}_{\mbf{x}\sim q} \mbb{E}_{p_\theta(\mbf{t}\mid\mbf{x})}[\partial_\mu\log p_\theta(\mbf{t}\mid\mbf{x})\partial_\nu \log p_\theta(\mbf{t}\mid\mbf{x})]$. Let the loss function $L(r_\theta) = - \mbb{E}_{\mbf{x}\sim q} [\log p_\theta(\mbf{l}\mid\mbf{x})]$ be the expected negative log-likelihood, where $\mbf{l}$ denotes the ground truth labels in the training dataset. Our learning goal is to find a model $r_{\theta^*}$ that minimizes the (empirical) loss $L(r_\theta)$.

The well known update rule of gradient descent $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda \partial_\mu L(r_{\theta_k})$ can be viewed as approximately solving the (continuous time) ODE
\begin{equation}
\dot\theta^\mu = -\lambda \partial_\mu L(r_\theta) \label{eqn:sgd}
\end{equation}
with forward Euler method. Here $\lambda$ is a time scale constant, $h$ is the step size, and their product $h\lambda$ is the learning rate. Note that $\lambda$ will only affect the ``speed'' but not trajectory of the system. It is notorious that the gradient descent ODE is not invariant to reparameterizations~\citep{ollivier2013riemannian,martens2010deep}. For example, if we rescale $\theta^\mu$ to $2 \theta^\mu$, $\partial_\mu L(r_\theta)$ will be downscaled to $\frac{1}{2} \partial_\mu L(r_\theta)$. This is more evident from a differential geometric point of view. As can be verified by chain rule, $\dot\theta^\mu$ transforms contravariantly and can therefore be treated as a vector in $\mcal{T}_p\mcal{M}$, while $\partial_\mu L(r_\theta)$ transforms covariantly, thus being a covector in $\mcal{T}^*_p\mcal{M}$. Because Eq.~\eqref{eqn:sgd} tries to relate objects in different spaces with different transformation rules, it is not an invariant relation.

Natural gradient alleviates this issue by approximately solving an invariant ODE. Recall that we can raise or lower an index given a metric tensor $g_{\mu\nu}$. By raising the index of $\partial_\mu L(r_\theta)$, the r.h.s. of the gradient descent ODE (Eq.~\eqref{eqn:sgd}) becomes a vector in $\mcal{T}_p\mcal{M}$, which solves the type mismatch problem of Eq.~\eqref{eqn:sgd}. The new ODE
\begin{equation}
\dot\theta^\mu = - \lambda g^{\mu\nu} \partial_\nu L(r_\theta) \label{eqn:ng}
\end{equation}
is now invariant, and the forward Euler approximation becomes $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda g^{\mu\nu}\partial_\nu L(r_{\theta_k})$, which is the traditional natural gradient update~\citep{amari1998natural}. 


%From the viewpoint of Riemannian geometry, natural gradient is fairly intuitive. Let the model manifold be $\mcal{M} := \{p_\theta(\mbf{z}), \theta\in\Theta\}$ equipped with the Fisher information metric $g_{\mu\nu} = (\mbf{F}_\theta)_{\mu\nu}$. We can view the parameterization using $\theta$ as a chart of $\mcal{M}$. The loss $l(p_\theta(\mbf{z}))$ is then a function on the manifold, and an optimization procedure implicitly defines trajectories on the manifold. When the learning rate is infinitesimal, gradient descent $\theta_{t+1} \gets \theta_t - \eta \nabla_{\theta_t}l(p_{\theta_t}(\mbf{z}))$ converges to a differential equation $\dot \theta^\mu = - \partial_\mu l$ as $\eta \rightarrow 0$. However, the equation does not type check, as $\dot \theta^\mu$ is a vector and $\partial_\mu l$ is a covector, which belong to different spaces ($\mcal{T}_p\mcal{M}$ and $\mcal{T}_p^* \mcal{M}$). Since vectors transform contravariantly and covectors transform covariantly, the equation will not be invariant to reparameterizations. Fortunately, as discussed in the previous section, the metric tensor $g_{\mu\nu}$ induces a natural map of a covector to a vector by raising indices. The corrected differential equation becomes $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$, which is exactly the natural gradient update under infinitesimal learning rate.

%Since $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$ is a relation between two vectors at the same tangent space, it is intrinsic to the model manifold and hence invariant to reparameterizations. However, an update rule with finite learning rate $\eta$ breaks this invariance property,
%Actually, $\theta_{t+1}^\mu \gets \theta_{t}^\mu - \eta g^{\mu\nu}\partial_\nu l$ is only invariant to affine transformations in flat spaces. Most model manifolds have non-vanishing curvatures
%and this update rule can only be viewed as an approximate solution to the invariant differential equation. 
%and can be viewed as an approximate solution to the invariant differential equation.
%Our main goal in this paper is demonstrating approaches and benefits of improving the invariance of natural gradient update.


==> ICML 2018 arXiv/preliminaries.tex <==
\section{Riemannian geometry and invariance}\label{sec:pre}
%In this section, we introduce notation conventions and some basic concepts in Riemannian geometry. We also provide an overview for natural gradient method.

%\subsection{Einstein's summation convention}
We use Einstein's summation convention throughout this paper to simplify formulas. The convention states that when any index variable appears twice in a term, once as a superscript and once as a subscript, it indicates summation of the term over all possible values of the index variable.
%, as long as the index is not otherwise defined. 
For example, $a^\mu b_\mu := \sum_{\mu=1}^n a^\mu b_\mu$ when index variable $\mu \in [n]$. We will write the summation symbol $\Sigma$ explicitly if we do not assume Einstein's summation convention on some index, \eg, $\sum_{\nu=1}^m a_\nu b_\nu c^\mu d_\mu := \sum_{\mu=1}^n \sum_{\nu=1}^m a_\nu b_\nu c^\mu d_\mu$.

%As an additional note, a free index variable in a formula indicates that the formula holds generally for any value of the variable, \eg, $\theta^\mu = \xi^\mu$ actually means $\forall \mu, \theta^\mu = \xi^\mu$. Also, we often identify a component of a tensor with the tensor itself, if the index is free. In other words, we use $\theta^\mu$ to denote the vector $\bs{\theta}$, $g_{\mu\nu}$ to denote the matrix $(g_{\mu\nu})$, \etc.

%\subsection{Riemannian geometry and invariance}
Riemannian geometry is used to study intrinsic properties of differentiable manifolds equipped with metrics. The goal of this necessarily brief section is to introduce some key concepts. For 
%a thorough review of the topic and its application to statistics, one can 
more details, please 
refer to~\cite{petersen2006riemannian} and~\cite{amari1987differential}.

\begin{figure}
	\centering
		\includegraphics[width=0.7\textwidth]{tangent_plane_plot.jpg}
	\caption{An illustration of tangent spaces, cotangent spaces, coordinate basis and dual coordinate basis, connection, parallel transportation, geodesics and the exponential map.}
	\label{fig:geometry}
\end{figure}

In this paper, we describe the space of some probabilistic models as a manifold. Informally, a \emph{manifold} $\mcal{M}$ of dimension $n$ is a smooth space whose local regions resemble $\mbb{R}^n$~\cite{carroll2004spacetime}. Smoothness allows us to define one-to-one smooth mapping $\phi: U \subset \mcal{M} \rightarrow \mbb{R}^n$ called \emph{chart} or \emph{coordinate system}, and for any $p\in U$, $\phi(p)$ represents the coordinates of $p$. For instance, if $p$ is a parameterized distribution, $\phi(p)$ will refer to its parameters. Generally, manifolds may need a group of charts for complete description.%A single chart is usually able to describe only a part of the manifold, but there exists a family of charts (called \emph{atlas}) that can cover the whole manifold, with all charts in the family ``compatible'' to each other on overlapping regions. For example, a sphere is a 2-dimensional manifold that can be covered using two charts via stereographic projections.

Local resemblance to $\mbb{R}^n$ provides the foundation for defining a linear space attached to each point $p \in \mcal{M}$ called the \emph{tangent space} $\mcal{T}_p\cal{M}$. Formally, $\mcal{T}_p\cal{M}$$=\{ \gamma'(0): \gamma \textrm{ is a smooth curve } \gamma:\mbb{R} \rightarrow \mcal{M},  \gamma(0)=p \}$ is the collection of all vectors obtained by differentiating smooth curves
through $p$, and consists of all tangent vectors to the manifold at point $p$. 
Each tangent vector $v \in \mcal{T}_p\cal{M}$ can be identified with a directional differential operator acting on 
functions defined on $\mcal{M}$, with direction $v$.
%It can be shown that $\mcal{T}_p\cal{M}$ is a vector space of dimension $n$, and a basis can be obtained as follows. 
Let $\phi(p) = (\theta^1,\theta^2,\cdots,\theta^n)$ be the coordinates of $p$, it can be shown that the set of operators $\{\frac{\partial}{\partial \theta^1},\cdots,\frac{\partial}{\partial \theta^n}\}$ forms a basis for $\mcal{T}_p\mcal{M}$ and is called the \emph{coordinate basis}. 
%Here the operator $\frac{\partial}{\partial \theta^\mu}$ applied to a function $f$ defined on $\cal{M}$ gives $\frac{\partial (f \circ \phi^{-1})}{\partial \theta^\mu}\rvert_{\phi(p)}$, and corresponds to the direction obtained by freezing all coordinates but the $\mu$-th coordinate at point $p$. 
Note that $\frac{\partial}{\partial \theta^\mu}$ is abbreviated to $\partial_\mu$ and $p$ is often identified with its coordinates $\theta^\mu$ in the sequel. 

Any vector space $V$ has a corresponding dual vector space $V^*$ consisting of all linear functionals on $V$. The dual vector space of $\mcal{T}_p\cal{M}$ is called the \emph{cotangent space} and is denoted $\mcal{T}_p^* \mcal{M}$.
% and consists of all linear forms on $\mcal{T}_p\cal{M}$. 
Because $\mcal{T}_p\cal{M}$ is finite-dimensional, $\mcal{T}_p^* \mcal{M}$ has the same dimension $n$ as $\mcal{T}_p\cal{M}$. $\mcal{T}_p^* \mcal{M}$ admits the \emph{dual coordinate basis} $\{\ud\theta^1,\cdots,\ud\theta^n\}$.
%Additionally, the dual of coordinate basis form the basis of $\mcal{T}_p^* \mcal{M}$, which is $\{\ud\theta^1,\cdots,\ud\theta^n\}$. 
These two sets of bases satisfy $\ud\theta^\mu(\partial_\nu) = \delta^\mu_\nu$ where $\delta^\mu_\nu$ is the Kronecker delta.
To gain some intuition, if $V$ is the space of all $n$-dimensional column vectors, $V^*$ can be identified with the space of $n$-dimensional row vectors.
%Another relevant example of dual spaces is the differential of a scalar function  $f$ defined on $\cal{M}$ (\eg, a loss function), which maps directional derivative operator to the corresponding directional derivative of $f$.
%Additionally, the dual of coordinate basis form the basis of $\mcal{T}_p^* \mcal{M}$, which is $\{\ud\theta^1,\cdots,\ud\theta^n\}$. These two sets of bases satisfy $\ud\theta^\mu(\partial_\nu) = \delta^\mu_\nu$.

Vectors and covectors are geometric objects which exist independently of the coordinate system. Their geometric properties do not depend on the basis used, however, their representation, in terms of coefficients, is of course basis dependent. In particular, a change in the coordinate system (\eg, corresponding to switching from cartesian to polar coordinates) around $p$ will alter the coordinate basis of $\mcal{T}_p\mcal{M}$, resulting in transformations of coefficients of both vectors and covectors. Let the new chart be $\phi'$ and let $\phi(p) = (\theta^1,\cdots,\theta^n), \phi'(p) = (\xi^1,\cdots,\xi^n)$. The new coefficients of $\mbf{a} \in \mcal{T}_p\mcal{M}$ will be given by 
$
a^{\mu'} \partial_{\mu'} = a^\mu \partial_\mu = a^\mu \frac{\partial \xi^{\mu'}}{\partial \theta^\mu} \partial_{\mu'} \Rightarrow a^{\mu'} = a^\mu \frac{\partial \xi^{\mu'}}{\partial \theta^\mu},
$
while the new coefficients of $\mbf{a}^* \in \mcal{T}_p^*\mcal{M}$ will be determined by 
$
a_{\mu'} \ud\xi^{\mu'} = a_\mu \ud\theta^\mu = a_\mu \frac{\partial \theta^\mu}{\partial \xi^{\mu'}} \ud\xi^{\mu'} \Rightarrow a_{\mu'} = a_\mu \frac{\partial \theta^\mu}{\partial \xi^{\mu'}}.
$
Due to the difference of transformation rules, we call $a^\mu$ to be \emph{contravariant} while $a_\mu$ \emph{covariant}, as indicated by superscripts and subscripts respectively. For example, imagine a constant rescaling of the coordinates, such that all the new basis vectors are scaled by $1/2$. To preserve the identity of a vector, its coefficients in this new basis will have to increase by a factor of $2$ (changing contra-variantly with respect to the basis vectors). This in turn means that the coefficients of a covector in the new basis will have to be scaled by $1/2$ (changing co-variantly), so that it yields the same result when applied to a vector whose coefficients are twice as large in the new basis.

Riemannian manifolds are those equipped with a positive definite metric tensor $g_p \in \mcal{T}_p^* \mcal{M} \otimes \mcal{T}_p^* \mcal{M}$. It is a symmetric bilinear positive definite scalar function of two vectors which defines the inner product structure of $\mcal{T}_p\mcal{M}$, and makes it possible to define geometric notions such as angles and lengths of curves.
Namely, the inner product of two vectors $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, $\mbf{b} = b^\nu \partial_\nu \in \mcal{T}_p\mcal{M}$ is defined as $\langle \mbf{a}, \mbf{b} \rangle := g_p(\mbf{a}, \mbf{b}) = g_{\mu\nu} \ud\theta^\mu \otimes \ud\theta^\nu (a^\mu \partial_\mu, b^\nu\partial_\nu) = g_{\mu\nu} a^\mu b^\nu$. Here we drop the subscript $p$ to avoid cluttering notations, although $g_{\mu\nu}$ can depend on $p$. For convenience, we denote the inverse of the metric tensor as $g^{\alpha\beta}$ using superscripts, \ie, $g^{\alpha\beta} g_{\beta\mu} = \delta^\alpha_\mu$.


The introduction of inner product induces a natural map from a tangent space to its dual. Let $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, its natural correspondence in $\mcal{T}_p^*\mcal{M}$ is the covector $\mbf{a}^* := \langle \mbf{a}, \cdot \rangle$. Let $\mbf{a}^* = a_\mu d\theta^\mu$, for any vector $\mbf{b} = b^\nu \partial_\nu \in \mcal{T}_p\mcal{M}$, we have $\langle \mbf{a}, \mbf{b}\rangle = a^\mu b^\nu g_{\mu\nu} = \mbf{a}^*(\mbf{b}) = a_\mu d\theta^\mu(b^\nu \partial_\nu) = a_\mu b^\nu \delta^\mu_\nu = a_\mu b^\mu = a_\nu b^\nu$. Since the equation holds for arbitrary $\mbf{b}$, we have $a_\nu = a^\mu g_{\mu\nu}$ and $a^\mu = g^{\mu\nu}a_\nu$. Therefore the metric tensor relates the coefficients of a vector and its covector by lowering and raising indices.


\begin{comment}
In order to compare tensors from two nearby tangent spaces $\mcal{T}_p\mcal{M}$ and $\mcal{T}_{p+dp}\mcal{M}$, we define the notion of a \emph{connection}. Let $m: \mcal{T}_{p+dp}\mcal{M} \rightarrow \mcal{T}_p\mcal{M}$. The vector
$
\nabla_{\mu} \partial_\nu = \lim_{\ud\bs{\theta}\rightarrow 0} \frac{\ud}{\ud\theta^\mu}[m(\partial_\nu') - \partial_\nu]
$
describes how fast the basis $\partial_\nu$ changes in the direction of $\partial_\mu$ as the point moves from $p$ to $p+dp$. The \emph{connection} $\Gamma_{\mu\nu}^\alpha$ is defined via $\nabla_{\mu} \partial_\nu = \Gamma_{\mu\nu}^\alpha \partial_\alpha$. Given the change rate of bases, the change rate of any vector $\mbf{a}$ along direction $\mbf{b}$ can be computed by
$
\nabla_{\mbf{b}} \mbf{a} = b^\mu \nabla_\mu (a^\nu \partial_\nu) = b^\mu (\partial_\mu a^\nu) \partial_\nu + b^\mu a^\nu \Gamma_{\mu\nu}^\alpha \partial_\alpha.
$
We can thus \emph{parallel transport} a vector $\mbf{a}$ along a curve $\theta(t)$ while preserving the vector in the sense of $\nabla_{\dot \theta} \mbf{a}(t) = 0$, where $\dot \theta = \frac{d\theta}{dt}$ represents the tangent vector of $\theta(t)$. There are some flexibilities in defining the connection. However, there exists a unique connection called \emph{Levi-Civita connection}, which can ensure geodesic lines to parallel transport their own tangent vectors. This gives the geodesic equation 
\begin{align}
\nabla_{\dot{\theta}} \dot{\theta} = 0 \Rightarrow \frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0,\label{eqn:geo}
\end{align} 
where the Levi-Civita connection here is the Christoffel symbol
\begin{align}
\Gamma_{\mu\nu}^\alpha = \frac{1}{2} g^{\alpha \beta}(\partial_\mu g_{\beta\nu} + \partial_\nu g_{\beta\mu} - \partial_\beta g_{\mu\nu}).\label{eqn:connection}
\end{align}
\end{comment}


Consider a curve $\gamma(t): I \rightarrow \mbb{R}^2$. Using Cartesian coordinates $\gamma(t)=(x(t),y(t))$, it is easy to verify that $\gamma$ is a straight line if it satisfies the following equation $\frac{\ud^2 x}{\ud t} =\frac{\ud^2 y}{\ud t}=0$, \ie, $x(t) = x_0 + v_x t, y(t) = y_0 + v_y t$. However, if we represent the curve using polar coordinates $\gamma(t)=(r(t),\theta(t))$, \ie, $x = r \cos \theta, y = r \sin \theta$, then $\frac{\ud^2 r}{\ud t} =\frac{\ud^2 \theta}{\ud t}=0$ does \emph{not} correspond to a straight line. The issue is that the coordinate basis depends on the position and will change as we move. For example, the radial directions $\partial r$ at two points on a circle will be different. 
%In general, we cannot meaningfully compare vectors from two nearby tangent spaces $\mcal{T}_p\mcal{M}$ and $\mcal{T}_{p+dp}\mcal{M}$ because they belong to different vector spaces. 
%To overcome this issue, we introduce the notion of a \emph{connection}.
We denote
$
\nabla_{\mu} \partial_\nu
$
the vector describing how fast the basis $\partial_\nu$ changes in the direction of $\partial_\mu$. %as the point moves from $p$ to $p+dp$. 
It is given by $\nabla_{\mu} \partial_\nu = \Gamma_{\mu\nu}^\alpha \partial_\alpha$ where $\Gamma_{\mu\nu}^\alpha$ is the \emph{connection}, which specifies additional manifold structure associated with curvature and parallelness. Here we use the Levi-Civita connection which is defined in terms of the metric as 
\begin{align}
\Gamma_{\mu\nu}^\alpha = \frac{1}{2} g^{\alpha \beta}(\partial_\mu g_{\beta\nu} + \partial_\nu g_{\beta\mu} - \partial_\beta g_{\mu\nu}).\label{eqn:connection}
\end{align}
A connection also specifies a way to transport a vector along a curve so that it stays parallel (to itself) with respect to the connection.
Given the change rate of bases specified by the connection, the change rate of any vector $\mbf{a}$ along direction $\mbf{b}$ can be computed by
$
\nabla_{\mbf{b}} \mbf{a} = b^\mu \nabla_\mu (a^\nu \partial_\nu) = b^\mu (\partial_\mu a^\nu) \partial_\nu + b^\mu a^\nu \Gamma_{\mu\nu}^\alpha \partial_\alpha.
$
We define the \emph{parallel transport} of a vector $\mbf{a}$ along a curve $\theta(t)$ as the solution to $\nabla_{\dot \theta} \mbf{a}(t) = 0$, where $\dot \theta = \frac{d\theta}{dt}$ represents the tangent vector of $\theta(t)$. This notion can be used to define the analogue of ``straight lines'', or geodesics, in general manifolds. A curve $\theta(t)$ is a geodesic 
%with parameter t 
if the tangent vector $\dot \theta = \frac{d\theta}{dt}$ is propagated parallelly to itself along the curve.
This gives the geodesic equation $\nabla_{\dot{\theta}} \dot{\theta} = 0$, or equivalently
\begin{align}
%\nabla_{\dot{\theta}} \dot{\theta} = 0 \Rightarrow \frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0\label{eqn:geo}
%\frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0.\label{eqn:geo}
\ddot\theta^\alpha + \Gamma_{\mu\nu}^\alpha \dot\theta^\mu \dot \theta^\nu = 0\label{eq:geo}
\end{align}
Note that  $\Gamma_{\mu\nu}^{\alpha}=0$ for $\mbb{R}^n$ with Euclidean metric and we recover usual straight lines. Let $v \in \mcal{T}_p\mcal{M}$, there exists a unique geodesic satisfying $\gamma(0)=p, \dot{\gamma}(0) = v$. This enables us to define the \emph{exponential map}, \ie, $\operatorname{Exp}(p,v) := \gamma(1)$. By simple scaling we also have $\operatorname{Exp}(p, h v) = \gamma(h)$. Consistent with our intuition, geodesics (\wrt Levi-Civia connection) also correspond to local shortest paths between two points. 

As a summary, we provide a graphical illustration of relevant concepts in Riemannian geometry in~\figref{fig:geometry}. From the above formulation, we observe that every concept and relation is defined via coordinates or coefficients. However, we need to discern the important ontological difference between an object and its coordinate. The manifold itself, along with geodesics and vectors (covectors) in its tangent (cotangent) spaces is intrinsic and independent of coordinates provided by charts. Riemannian geometry studies intrinsic properties of manifolds via the lens of coordinates. As long as the coordinates are transformed accordingly, \eg, both transforms covariantly or contravariantly, the objects and their relations will not change. This is where invariance emerges.

\section{Natural gradient method}
Let $r_\theta(\mbf{z}) = p_\theta(\mbf{t}\mid\mbf{x})q(\mbf{x})$ be a probabilistic model parameterized by $\theta \in \Theta$, and $L(r_\theta) = - \mbb{E}_{\mbf{x}\sim q} [\log p_\theta(\mbf{t}\mid\mbf{x})]$ be the expected negative log-likelihood. Here $\mbf{x},\mbf{t}$ are random variables, $\mbf{z} = (\mbf{x},\mbf{t})$ is their joint, $q(\mbf{x})$ is the marginal distribution of $\mbf{x}$ and is independent of $\theta$. In a Riemannian geometry framework, the set of all possible models $r_\theta$ constitutes a manifold $\mcal{M}$, and the parameter $\theta$ provides a chart. Our goal is to find a model $r_{\theta^*}$ that minimizes the (empirical) loss $L(r_\theta)$, which is a function defined on the manifold. %Note that every component in this task definition depends only on the manifold and should be invariant to all parameterizations.

The well known update rule of gradient descent $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda \partial_\mu L(r_{\theta_k})$ can be viewed as approximately solving the ordinary differential equation (ODE) $\dot\theta^\mu = -\lambda \partial_\mu L(r_\theta)$ with forward Euler method. Here $\lambda$ is a time scale constant, $h$ is the step size, and their product $h\lambda$ is the learning rate. However, the gradient descent ODE is not invariant to reparameterizations. For example, if we rescale $\theta^\mu$ to $2 \theta^\mu$, $\partial_\mu L(r_\theta)$ will be downscaled to $\frac{1}{2} \partial_\mu L(r_\theta)$. This is more evident from a differential geometric point of view. As can be verified by chain rules, $\dot\theta^\mu$ transforms contravariantly and therefore is a vector in $\mcal{T}_p\mcal{M}$, while $\partial_\mu L(r_\theta)$ transforms covariantly, thus being a covector in $\mcal{T}^*_p\mcal{M}$. Accordingly, the l.h.s. and r.h.s. of the ODE transform with different rules and do not type check. As a result, optimizing $L(r_\theta)$ with gradient descent is using a parameterization-dependent method to solve a parameterization-independent problem, which is aesthetically unsatisfying.
%depends on the model $p_\theta(\mbf{z})$, while being agnostic to a specific parameterization.
%Linear scaling already has a big impact on the performance of gradient descent, let alone more complicated nonlinear parameter transformations. As a consequence, it would be beneficial to have the optimization problem depend only on the model $p_\theta(\mbf{z})$, while being agnostic to a specific parameterization.

Natural gradient alleviates this issue by approximately solving an invariant ODE. Recall that we can raise or lower an index given a metric tensor $g_{\mu\nu}$, and hereby we choose the Fisher information metric given by $g_{\mu\nu} = \mbb{E}_{\mbf{x}\sim q} \mbb{E}_{p_\theta(\mbf{t}\mid\mbf{x})}[\partial_\mu\log p_\theta(\mbf{t}\mid\mbf{x})\partial_\nu \log p_\theta(\mbf{t}\mid\mbf{x})]$. By raising the index of $\partial_\mu L(r_\theta)$, the r.h.s. of the gradient descent ODE becomes a vector in $\mcal{T}_p\mcal{M}$ and both sides transform contravariantly. The new invariant ODE is now $\dot\theta^\mu = - \lambda g^{\mu\nu} \partial_\nu L(r_\theta)$, and the forward Euler approximation becomes $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda g^{\mu\nu}\partial_\nu L(r_{\theta_k})$, which is the traditional natural gradient update~\cite{amari1998natural}. 

\begin{comment}
From the viewpoint of Riemannian geometry, natural gradient is fairly intuitive. Let the model manifold be $\mcal{M} := \{p_\theta(\mbf{z}), \theta\in\Theta\}$ equipped with the Fisher information metric $g_{\mu\nu} = (\mbf{F}_\theta)_{\mu\nu}$. We can view the parameterization using $\theta$ as a chart of $\mcal{M}$. The loss $l(p_\theta(\mbf{z}))$ is then a function on the manifold, and an optimization procedure implicitly defines trajectories on the manifold. When the learning rate is infinitesimal, gradient descent $\theta_{t+1} \gets \theta_t - \eta \nabla_{\theta_t}l(p_{\theta_t}(\mbf{z}))$ converges to a differential equation $\dot \theta^\mu = - \partial_\mu l$ as $\eta \rightarrow 0$. However, the equation does not type check, as $\dot \theta^\mu$ is a vector and $\partial_\mu l$ is a covector, which belong to different spaces ($\mcal{T}_p\mcal{M}$ and $\mcal{T}_p^* \mcal{M}$). Since vectors transform contravariantly and covectors transform covariantly, the equation will not be invariant to reparameterizations. Fortunately, as discussed in the previous section, the metric tensor $g_{\mu\nu}$ induces a natural map of a covector to a vector by raising indices. The corrected differential equation becomes $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$, which is exactly the natural gradient update under infinitesimal learning rate.

Since $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$ is a relation between two vectors at the same tangent space, it is intrinsic to the model manifold and hence invariant to reparameterizations. However, an update rule with finite learning rate $\eta$ breaks this invariance property,
%Actually, $\theta_{t+1}^\mu \gets \theta_{t}^\mu - \eta g^{\mu\nu}\partial_\nu l$ is only invariant to affine transformations in flat spaces. Most model manifolds have non-vanishing curvatures
%and this update rule can only be viewed as an approximate solution to the invariant differential equation. 
and can be viewed as an approximate solution to the invariant differential equation.
Our main goal in this paper is demonstrating approaches and benefits of improving the invariance of natural gradient update.
\end{comment}

==> preliminaries.tex <==
\section{Riemannian geometry and invariance}\label{sec:pre}
%In this section, we introduce notation conventions and some basic concepts in Riemannian geometry. We also provide an overview for natural gradient method.

%\subsection{Einstein's summation convention}
We use Einstein's summation convention throughout this paper to simplify formulas. The convention states that when any index variable appears twice in a term, once as a superscript and once as a subscript, it indicates summation of the term over all possible values of the index variable.
%, as long as the index is not otherwise defined. 
For example, $a^\mu b_\mu := \sum_{\mu=1}^n a^\mu b_\mu$ when index variable $\mu \in [n]$. We will write the summation symbol $\Sigma$ explicitly if we do not assume Einstein's summation convention on some index, \eg, $\sum_{\nu=1}^m a_\nu b_\nu c^\mu d_\mu := \sum_{\mu=1}^n \sum_{\nu=1}^m a_\nu b_\nu c^\mu d_\mu$.

%As an additional note, a free index variable in a formula indicates that the formula holds generally for any value of the variable, \eg, $\theta^\mu = \xi^\mu$ actually means $\forall \mu, \theta^\mu = \xi^\mu$. Also, we often identify a component of a tensor with the tensor itself, if the index is free. In other words, we use $\theta^\mu$ to denote the vector $\bs{\theta}$, $g_{\mu\nu}$ to denote the matrix $(g_{\mu\nu})$, \etc.

%\subsection{Riemannian geometry and invariance}
Riemannian geometry is used to study intrinsic properties of differentiable manifolds equipped with metrics. The goal of this necessarily brief section is to introduce some key concepts. For 
%a thorough review of the topic and its application to statistics, one can 
more details, please 
refer to~\cite{petersen2006riemannian} and~\cite{amari1987differential}.

\begin{figure}
	\centering
		\includegraphics[width=0.7\textwidth]{tangent_plane_plot.jpg}
	\caption{An illustration of tangent spaces, cotangent spaces, coordinate basis and dual coordinate basis, connection, parallel transportation, geodesics and the exponential map.}
	\label{fig:geometry}
\end{figure}

In this paper, we describe the space of some probabilistic models as a manifold. Informally, a \emph{manifold} $\mcal{M}$ of dimension $n$ is a smooth space whose local regions resemble $\mbb{R}^n$~\cite{carroll2004spacetime}. Smoothness allows us to define one-to-one smooth mapping $\phi: U \subset \mcal{M} \rightarrow \mbb{R}^n$ called \emph{chart} or \emph{coordinate system}, and for any $p\in U$, $\phi(p)$ represents the coordinates of $p$. For instance, if $p$ is a parameterized distribution, $\phi(p)$ will refer to its parameters. Generally, manifolds may need a group of charts for complete description.%A single chart is usually able to describe only a part of the manifold, but there exists a family of charts (called \emph{atlas}) that can cover the whole manifold, with all charts in the family ``compatible'' to each other on overlapping regions. For example, a sphere is a 2-dimensional manifold that can be covered using two charts via stereographic projections.

Local resemblance to $\mbb{R}^n$ provides the foundation for defining a linear space attached to each point $p \in \mcal{M}$ called the \emph{tangent space} $\mcal{T}_p\cal{M}$. Formally, $\mcal{T}_p\cal{M}$$=\{ \gamma'(0): \gamma \textrm{ is a smooth curve } \gamma:\mbb{R} \rightarrow \mcal{M},  \gamma(0)=p \}$ is the collection of all vectors obtained by differentiating smooth curves
through $p$, and consists of all tangent vectors to the manifold at point $p$. 
Each tangent vector $v \in \mcal{T}_p\cal{M}$ can be identified with a directional differential operator acting on 
functions defined on $\mcal{M}$, with direction $v$.
%It can be shown that $\mcal{T}_p\cal{M}$ is a vector space of dimension $n$, and a basis can be obtained as follows. 
Let $\phi(p) = (\theta^1,\theta^2,\cdots,\theta^n)$ be the coordinates of $p$, it can be shown that the set of operators $\{\frac{\partial}{\partial \theta^1},\cdots,\frac{\partial}{\partial \theta^n}\}$ forms a basis for $\mcal{T}_p\mcal{M}$ and is called the \emph{coordinate basis}. 
%Here the operator $\frac{\partial}{\partial \theta^\mu}$ applied to a function $f$ defined on $\cal{M}$ gives $\frac{\partial (f \circ \phi^{-1})}{\partial \theta^\mu}\rvert_{\phi(p)}$, and corresponds to the direction obtained by freezing all coordinates but the $\mu$-th coordinate at point $p$. 
Note that $\frac{\partial}{\partial \theta^\mu}$ is abbreviated to $\partial_\mu$ and $p$ is often identified with its coordinates $\theta^\mu$ in the sequel. 

Any vector space $V$ has a corresponding dual vector space $V^*$ consisting of all linear functionals on $V$. The dual vector space of $\mcal{T}_p\cal{M}$ is called the \emph{cotangent space} and is denoted $\mcal{T}_p^* \mcal{M}$.
% and consists of all linear forms on $\mcal{T}_p\cal{M}$. 
Because $\mcal{T}_p\cal{M}$ is finite-dimensional, $\mcal{T}_p^* \mcal{M}$ has the same dimension $n$ as $\mcal{T}_p\cal{M}$. $\mcal{T}_p^* \mcal{M}$ admits the \emph{dual coordinate basis} $\{\ud\theta^1,\cdots,\ud\theta^n\}$.
%Additionally, the dual of coordinate basis form the basis of $\mcal{T}_p^* \mcal{M}$, which is $\{\ud\theta^1,\cdots,\ud\theta^n\}$. 
These two sets of bases satisfy $\ud\theta^\mu(\partial_\nu) = \delta^\mu_\nu$ where $\delta^\mu_\nu$ is the Kronecker delta.
To gain some intuition, if $V$ is the space of all $n$-dimensional column vectors, $V^*$ can be identified with the space of $n$-dimensional row vectors.
%Another relevant example of dual spaces is the differential of a scalar function  $f$ defined on $\cal{M}$ (\eg, a loss function), which maps directional derivative operator to the corresponding directional derivative of $f$.
%Additionally, the dual of coordinate basis form the basis of $\mcal{T}_p^* \mcal{M}$, which is $\{\ud\theta^1,\cdots,\ud\theta^n\}$. These two sets of bases satisfy $\ud\theta^\mu(\partial_\nu) = \delta^\mu_\nu$.

Vectors and covectors are geometric objects which exist independently of the coordinate system. Their geometric properties do not depend on the basis used, however, their representation, in terms of coefficients, is of course basis dependent. In particular, a change in the coordinate system (\eg, corresponding to switching from cartesian to polar coordinates) around $p$ will alter the coordinate basis of $\mcal{T}_p\mcal{M}$, resulting in transformations of coefficients of both vectors and covectors. Let the new chart be $\phi'$ and let $\phi(p) = (\theta^1,\cdots,\theta^n), \phi'(p) = (\xi^1,\cdots,\xi^n)$. The new coefficients of $\mbf{a} \in \mcal{T}_p\mcal{M}$ will be given by 
$
a^{\mu'} \partial_{\mu'} = a^\mu \partial_\mu = a^\mu \frac{\partial \xi^{\mu'}}{\partial \theta^\mu} \partial_{\mu'} \Rightarrow a^{\mu'} = a^\mu \frac{\partial \xi^{\mu'}}{\partial \theta^\mu},
$
while the new coefficients of $\mbf{a}^* \in \mcal{T}_p^*\mcal{M}$ will be determined by 
$
a_{\mu'} \ud\xi^{\mu'} = a_\mu \ud\theta^\mu = a_\mu \frac{\partial \theta^\mu}{\partial \xi^{\mu'}} \ud\xi^{\mu'} \Rightarrow a_{\mu'} = a_\mu \frac{\partial \theta^\mu}{\partial \xi^{\mu'}}.
$
Due to the difference of transformation rules, we call $a^\mu$ to be \emph{contravariant} while $a_\mu$ \emph{covariant}, as indicated by superscripts and subscripts respectively. For example, imagine a constant rescaling of the coordinates, such that all the new basis vectors are scaled by $1/2$. To preserve the identity of a vector, its coefficients in this new basis will have to increase by a factor of $2$ (changing contra-variantly with respect to the basis vectors). This in turn means that the coefficients of a covector in the new basis will have to be scaled by $1/2$ (changing co-variantly), so that it yields the same result when applied to a vector whose coefficients are twice as large in the new basis.

Riemannian manifolds are those equipped with a positive definite metric tensor $g_p \in \mcal{T}_p^* \mcal{M} \otimes \mcal{T}_p^* \mcal{M}$. It is a symmetric bilinear positive definite scalar function of two vectors which defines the inner product structure of $\mcal{T}_p\mcal{M}$, and makes it possible to define geometric notions such as angles and lengths of curves.
Namely, the inner product of two vectors $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, $\mbf{b} = b^\nu \partial_\nu \in \mcal{T}_p\mcal{M}$ is defined as $\langle \mbf{a}, \mbf{b} \rangle := g_p(\mbf{a}, \mbf{b}) = g_{\mu\nu} \ud\theta^\mu \otimes \ud\theta^\nu (a^\mu \partial_\mu, b^\nu\partial_\nu) = g_{\mu\nu} a^\mu b^\nu$. Here we drop the subscript $p$ to avoid cluttering notations, although $g_{\mu\nu}$ can depend on $p$. For convenience, we denote the inverse of the metric tensor as $g^{\alpha\beta}$ using superscripts, \ie, $g^{\alpha\beta} g_{\beta\mu} = \delta^\alpha_\mu$.


The introduction of inner product induces a natural map from a tangent space to its dual. Let $\mbf{a} = a^\mu \partial_\mu \in \mcal{T}_p\mcal{M}$, its natural correspondence in $\mcal{T}_p^*\mcal{M}$ is the covector $\mbf{a}^* := \langle \mbf{a}, \cdot \rangle$. Let $\mbf{a}^* = a_\mu d\theta^\mu$, for any vector $\mbf{b} = b^\nu \partial_\nu \in \mcal{T}_p\mcal{M}$, we have $\langle \mbf{a}, \mbf{b}\rangle = a^\mu b^\nu g_{\mu\nu} = \mbf{a}^*(\mbf{b}) = a_\mu d\theta^\mu(b^\nu \partial_\nu) = a_\mu b^\nu \delta^\mu_\nu = a_\mu b^\mu = a_\nu b^\nu$. Since the equation holds for arbitrary $\mbf{b}$, we have $a_\nu = a^\mu g_{\mu\nu}$ and $a^\mu = g^{\mu\nu}a_\nu$. Therefore the metric tensor relates the coefficients of a vector and its covector by lowering and raising indices.


\begin{comment}
In order to compare tensors from two nearby tangent spaces $\mcal{T}_p\mcal{M}$ and $\mcal{T}_{p+dp}\mcal{M}$, we define the notion of a \emph{connection}. Let $m: \mcal{T}_{p+dp}\mcal{M} \rightarrow \mcal{T}_p\mcal{M}$. The vector
$
\nabla_{\mu} \partial_\nu = \lim_{\ud\bs{\theta}\rightarrow 0} \frac{\ud}{\ud\theta^\mu}[m(\partial_\nu') - \partial_\nu]
$
describes how fast the basis $\partial_\nu$ changes in the direction of $\partial_\mu$ as the point moves from $p$ to $p+dp$. The \emph{connection} $\Gamma_{\mu\nu}^\alpha$ is defined via $\nabla_{\mu} \partial_\nu = \Gamma_{\mu\nu}^\alpha \partial_\alpha$. Given the change rate of bases, the change rate of any vector $\mbf{a}$ along direction $\mbf{b}$ can be computed by
$
\nabla_{\mbf{b}} \mbf{a} = b^\mu \nabla_\mu (a^\nu \partial_\nu) = b^\mu (\partial_\mu a^\nu) \partial_\nu + b^\mu a^\nu \Gamma_{\mu\nu}^\alpha \partial_\alpha.
$
We can thus \emph{parallel transport} a vector $\mbf{a}$ along a curve $\theta(t)$ while preserving the vector in the sense of $\nabla_{\dot \theta} \mbf{a}(t) = 0$, where $\dot \theta = \frac{d\theta}{dt}$ represents the tangent vector of $\theta(t)$. There are some flexibilities in defining the connection. However, there exists a unique connection called \emph{Levi-Civita connection}, which can ensure geodesic lines to parallel transport their own tangent vectors. This gives the geodesic equation 
\begin{align}
\nabla_{\dot{\theta}} \dot{\theta} = 0 \Rightarrow \frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0,\label{eqn:geo}
\end{align} 
where the Levi-Civita connection here is the Christoffel symbol
\begin{align}
\Gamma_{\mu\nu}^\alpha = \frac{1}{2} g^{\alpha \beta}(\partial_\mu g_{\beta\nu} + \partial_\nu g_{\beta\mu} - \partial_\beta g_{\mu\nu}).\label{eqn:connection}
\end{align}
\end{comment}


Consider a curve $\gamma(t): I \rightarrow \mbb{R}^2$. Using Cartesian coordinates $\gamma(t)=(x(t),y(t))$, it is easy to verify that $\gamma$ is a straight line if it satisfies the following equation $\frac{\ud^2 x}{\ud t} =\frac{\ud^2 y}{\ud t}=0$, \ie, $x(t) = x_0 + v_x t, y(t) = y_0 + v_y t$. However, if we represent the curve using polar coordinates $\gamma(t)=(r(t),\theta(t))$, \ie, $x = r \cos \theta, y = r \sin \theta$, then $\frac{\ud^2 r}{\ud t} =\frac{\ud^2 \theta}{\ud t}=0$ does \emph{not} correspond to a straight line. The issue is that the coordinate basis depends on the position and will change as we move. For example, the radial directions $\partial r$ at two points on a circle will be different. 
%In general, we cannot meaningfully compare vectors from two nearby tangent spaces $\mcal{T}_p\mcal{M}$ and $\mcal{T}_{p+dp}\mcal{M}$ because they belong to different vector spaces. 
%To overcome this issue, we introduce the notion of a \emph{connection}.
We denote
$
\nabla_{\mu} \partial_\nu
$
the vector describing how fast the basis $\partial_\nu$ changes in the direction of $\partial_\mu$. %as the point moves from $p$ to $p+dp$. 
It is given by $\nabla_{\mu} \partial_\nu = \Gamma_{\mu\nu}^\alpha \partial_\alpha$ where $\Gamma_{\mu\nu}^\alpha$ is the \emph{connection}, which specifies additional manifold structure associated with curvature and parallelness. Here we use the Levi-Civita connection which is defined in terms of the metric as 
\begin{align}
\Gamma_{\mu\nu}^\alpha = \frac{1}{2} g^{\alpha \beta}(\partial_\mu g_{\beta\nu} + \partial_\nu g_{\beta\mu} - \partial_\beta g_{\mu\nu}).\label{eqn:connection}
\end{align}
A connection also specifies a way to transport a vector along a curve so that it stays parallel (to itself) with respect to the connection.
Given the change rate of bases specified by the connection, the change rate of any vector $\mbf{a}$ along direction $\mbf{b}$ can be computed by
$
\nabla_{\mbf{b}} \mbf{a} = b^\mu \nabla_\mu (a^\nu \partial_\nu) = b^\mu (\partial_\mu a^\nu) \partial_\nu + b^\mu a^\nu \Gamma_{\mu\nu}^\alpha \partial_\alpha.
$
We define the \emph{parallel transport} of a vector $\mbf{a}$ along a curve $\theta(t)$ as the solution to $\nabla_{\dot \theta} \mbf{a}(t) = 0$, where $\dot \theta = \frac{d\theta}{dt}$ represents the tangent vector of $\theta(t)$. This notion can be used to define the analogue of ``straight lines'', or geodesics, in general manifolds. A curve $\theta(t)$ is a geodesic 
%with parameter t 
if the tangent vector $\dot \theta = \frac{d\theta}{dt}$ is propagated parallelly to itself along the curve.
This gives the geodesic equation $\nabla_{\dot{\theta}} \dot{\theta} = 0$, or equivalently
\begin{align}
%\nabla_{\dot{\theta}} \dot{\theta} = 0 \Rightarrow \frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0\label{eqn:geo}
%\frac{\ud^2\theta^\alpha}{\ud t} + \Gamma_{\mu\nu}^{\alpha} \frac{\ud\theta^\mu}{\ud t} \frac{\ud\theta^\nu}{\ud t} = 0.\label{eqn:geo}
\ddot\theta^\alpha + \Gamma_{\mu\nu}^\alpha \dot\theta^\mu \dot \theta^\nu = 0\label{eq:geo}
\end{align}
Note that  $\Gamma_{\mu\nu}^{\alpha}=0$ for $\mbb{R}^n$ with Euclidean metric and we recover usual straight lines. Let $v \in \mcal{T}_p\mcal{M}$, there exists a unique geodesic satisfying $\gamma(0)=p, \dot{\gamma}(0) = v$. This enables us to define the \emph{exponential map}, \ie, $\operatorname{Exp}(p,v) := \gamma(1)$. By simple scaling we also have $\operatorname{Exp}(p, h v) = \gamma(h)$. Consistent with our intuition, geodesics (\wrt Levi-Civia connection) also correspond to local shortest paths between two points. 

As a summary, we provide a graphical illustration of relevant concepts in Riemannian geometry in~\figref{fig:geometry}. From the above formulation, we observe that every concept and relation is defined via coordinates or coefficients. However, we need to discern the important ontological difference between an object and its coordinate. The manifold itself, along with geodesics and vectors (covectors) in its tangent (cotangent) spaces is intrinsic and independent of coordinates provided by charts. Riemannian geometry studies intrinsic properties of manifolds via the lens of coordinates. As long as the coordinates are transformed accordingly, \eg, both transforms covariantly or contravariantly, the objects and their relations will not change. This is where invariance emerges.

\section{Natural gradient method}
Let $r_\theta(\mbf{z}) = p_\theta(\mbf{t}\mid\mbf{x})q(\mbf{x})$ be a probabilistic model parameterized by $\theta \in \Theta$, and $L(r_\theta) = - \mbb{E}_{\mbf{x}\sim q} [\log p_\theta(\mbf{t}\mid\mbf{x})]$ be the expected negative log-likelihood. Here $\mbf{x},\mbf{t}$ are random variables, $\mbf{z} = (\mbf{x},\mbf{t})$ is their joint, $q(\mbf{x})$ is the marginal distribution of $\mbf{x}$ and is independent of $\theta$. In a Riemannian geometry framework, the set of all possible models $r_\theta$ constitutes a manifold $\mcal{M}$, and the parameter $\theta$ provides a chart. Our goal is to find a model $r_{\theta^*}$ that minimizes the (empirical) loss $L(r_\theta)$, which is a function defined on the manifold. %Note that every component in this task definition depends only on the manifold and should be invariant to all parameterizations.

The well known update rule of gradient descent $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda \partial_\mu L(r_{\theta_k})$ can be viewed as approximately solving the ordinary differential equation (ODE) $\dot\theta^\mu = -\lambda \partial_\mu L(r_\theta)$ with forward Euler method. Here $\lambda$ is a time scale constant, $h$ is the step size, and their product $h\lambda$ is the learning rate. However, the gradient descent ODE is not invariant to reparameterizations. For example, if we rescale $\theta^\mu$ to $2 \theta^\mu$, $\partial_\mu L(r_\theta)$ will be downscaled to $\frac{1}{2} \partial_\mu L(r_\theta)$. This is more evident from a differential geometric point of view. As can be verified by chain rules, $\dot\theta^\mu$ transforms contravariantly and therefore is a vector in $\mcal{T}_p\mcal{M}$, while $\partial_\mu L(r_\theta)$ transforms covariantly, thus being a covector in $\mcal{T}^*_p\mcal{M}$. Accordingly, the l.h.s. and r.h.s. of the ODE transform with different rules and do not type check. As a result, optimizing $L(r_\theta)$ with gradient descent is using a parameterization-dependent method to solve a parameterization-independent problem, which is aesthetically unsatisfying.
%depends on the model $p_\theta(\mbf{z})$, while being agnostic to a specific parameterization.
%Linear scaling already has a big impact on the performance of gradient descent, let alone more complicated nonlinear parameter transformations. As a consequence, it would be beneficial to have the optimization problem depend only on the model $p_\theta(\mbf{z})$, while being agnostic to a specific parameterization.

Natural gradient alleviates this issue by approximately solving an invariant ODE. Recall that we can raise or lower an index given a metric tensor $g_{\mu\nu}$, and hereby we choose the Fisher information metric given by $g_{\mu\nu} = \mbb{E}_{\mbf{x}\sim q} \mbb{E}_{p_\theta(\mbf{t}\mid\mbf{x})}[\partial_\mu\log p_\theta(\mbf{t}\mid\mbf{x})\partial_\nu \log p_\theta(\mbf{t}\mid\mbf{x})]$. By raising the index of $\partial_\mu L(r_\theta)$, the r.h.s. of the gradient descent ODE becomes a vector in $\mcal{T}_p\mcal{M}$ and both sides transform contravariantly. The new invariant ODE is now $\dot\theta^\mu = - \lambda g^{\mu\nu} \partial_\nu L(r_\theta)$, and the forward Euler approximation becomes $\theta_{k+1}^\mu = \theta_k^\mu - h \lambda g^{\mu\nu}\partial_\nu L(r_{\theta_k})$, which is the traditional natural gradient update~\cite{amari1998natural}. 

\begin{comment}
From the viewpoint of Riemannian geometry, natural gradient is fairly intuitive. Let the model manifold be $\mcal{M} := \{p_\theta(\mbf{z}), \theta\in\Theta\}$ equipped with the Fisher information metric $g_{\mu\nu} = (\mbf{F}_\theta)_{\mu\nu}$. We can view the parameterization using $\theta$ as a chart of $\mcal{M}$. The loss $l(p_\theta(\mbf{z}))$ is then a function on the manifold, and an optimization procedure implicitly defines trajectories on the manifold. When the learning rate is infinitesimal, gradient descent $\theta_{t+1} \gets \theta_t - \eta \nabla_{\theta_t}l(p_{\theta_t}(\mbf{z}))$ converges to a differential equation $\dot \theta^\mu = - \partial_\mu l$ as $\eta \rightarrow 0$. However, the equation does not type check, as $\dot \theta^\mu$ is a vector and $\partial_\mu l$ is a covector, which belong to different spaces ($\mcal{T}_p\mcal{M}$ and $\mcal{T}_p^* \mcal{M}$). Since vectors transform contravariantly and covectors transform covariantly, the equation will not be invariant to reparameterizations. Fortunately, as discussed in the previous section, the metric tensor $g_{\mu\nu}$ induces a natural map of a covector to a vector by raising indices. The corrected differential equation becomes $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$, which is exactly the natural gradient update under infinitesimal learning rate.

Since $\dot \theta^\mu =  - g^{\mu\nu}\partial_\nu l$ is a relation between two vectors at the same tangent space, it is intrinsic to the model manifold and hence invariant to reparameterizations. However, an update rule with finite learning rate $\eta$ breaks this invariance property,
%Actually, $\theta_{t+1}^\mu \gets \theta_{t}^\mu - \eta g^{\mu\nu}\partial_\nu l$ is only invariant to affine transformations in flat spaces. Most model manifolds have non-vanishing curvatures
%and this update rule can only be viewed as an approximate solution to the invariant differential equation. 
and can be viewed as an approximate solution to the invariant differential equation.
Our main goal in this paper is demonstrating approaches and benefits of improving the invariance of natural gradient update.
\end{comment}
